Random 2D linear cocycles I: dichotomic behavior

In this paper we establish a Bochi-Ma\~n\'e type dichotomy in the space of two dimensional, nonnegative determinant matrix valued, locally constant linear cocycles over a Bernoulli or Markov shift. Moreover, we prove that Lebesgue almost every such cocycle has finite first Lyapunov exponent, which then implies a break in the regularity of the Lyapunov exponent, from analyticity to discontinuity.

==> applications.tex <==


aaa





==> ldt.tex <==
{\color{blue} Given the alphabet (set of symbols) $\Ascr = \{1, \ldots, k\}$ and a partition $\Ascr = \Asing \sqcup \Ainv$ into two nonempty sets, consider the space $\cocycles$ of all $k$-tuples $\underline{A} = (A_1, \ldots, A_k) \in \Mat_2 (\R)$ such that $\rank A_i = 1$ if $i \in \Asing$, $\rank A_j = 2$ if $j\in\Ainv$ and there are no null words, that is,  $A_{i_1} \cdots A_{i_l} \neq 0$ for all $l\in \N$ and $i_1, \ldots, i_l \in \Ascr$.

We identify such a $k$-tuple $\underline{A} = (A_1, \ldots, A_k)$ with the locally constant map $A \colon X \to \Mat_2 (\R)$, $A (\om) = A_{\om_0}$, where $\om = \{\om_n\}_{n\in \Z} \in X = \Ascr^\Z$, and we use these notations interchangeably.

Given a probability vector $p = (p_1, \ldots, p_k)$ with $p_i > 0$ for all $i$, each  $k$-tuple $\underline{A} = (A_1, \ldots, A_k)$ determines the random linear cocycle 
$F \colon X \times \R^2 \to X \times \R^2$,
$$F (\om, v) = (\sigma \om, A (\om) v) = (\sigma \om, A_{\om_0} \, v) \, ,$$
where $X$ is endowed with the product probability $\mu = p^\Z$.
We may also identify this cocycle with the tuple $\underline{A} = (A_1, \ldots, A_k)$.




Let $\Lambda \subset \R$ be a compact interval (normalized to have length $1$)  and let $A\colon \Lambda \to \cocycles$ be a smooth map. We think of this map as a one-parameter family of random cocycles so we use the subscrpt notation $t \mapsto A_t$. For its components we write $A_t (i)$ instead of $(A_t)_i$, while the fiber iterates are denoted by
$$A_t^n (\om) = A_t (\om_{n-1}) \cdots A_t (\om_0) \, .$$


\subsection*{Assumptions} We impose the following conditions on the smooth map  $t \mapsto A_t$.
\begin{enumerate}
\item[(A1)] For all $i\in \Asing$, $A_t (i) \equiv A_i$.

\item[(A2)] There is $c > 0$ such that for all $t \in \Lambda$, $j \in \Ainv$ and $\hat v \in \Proj$ we have
$$\frac{d}{d t} \, \frac{A_t (j) v}{\norm{A_t (j) v}} \ge c \, .$$
\end{enumerate}

\begin{example}
Given any tuple $\underline{A} = (A_1, \ldots, A_k) \in \cocycles$, the one-parameter family $\left[ - \frac{1}{2}, \frac{1}{2} \right] \mapsto A_t \in \Mat_2 (\R)^k$,
$A_t (i) = A_i$ if $i \in \Asing$ and 
$$A_t (j) = A_j \, R_{2 \pi t} = \begin{bmatrix} \cos 2 \pi t & - \sin 2 \pi t \\ \sin 2 \pi t & \cos 2 \pi t \end{bmatrix} \quad \text{if } \, j \in \Ainv $$
satisfies the assumptions (A1) and (A2) above and passes through $\underline{A}$.
\end{example}
 
\begin{theorem}(Abstract)
If $\underline{A}=(A_1,...,A_k)\in (\GL_2(\mathbb{R}))^k$ and $L_1(\underline{A})>L_2(\underline{A})$.
Then there exists a neighborhood $\mathcal{V}$ of $\underline{A}\in \GL_2(\mathbb{R})^k$ and $\exists a,b>0$ $\exists n_0$ such that $\forall n\geq n_0$

$$\mathbb{P}\bigg[\abs{\frac{1}{n}\log\norm{B^nv}-L_1(B)}>n^{-a}\bigg]\lesssim e^{-n^b}, \forall B\in\mathcal{V}.$$ 
\end{theorem}

\begin{theorem}
$\exists \Omega\subseteq \Lambda$ such that $Leb(\Lambda\setminus \Omega)=0$ and $\forall t\in\Omega$ $L_1(\underline{A}(t))>L_2(\underline{A}(t))\geq-\infty$. Also $\exists a,b>0$ and $n_0=n_0(t,a,b)$ such that $\forall n\geq n_0$ $$\mathbb{P}\bigg[\abs{\frac{1}{n}\log\norm{\underline{A}^nv}-L_1(\underline{A}(t))}>n^{-a}\bigg]\lesssim e^{-n^b}.$$
\end{theorem}

\begin{proof}
Notice that $\mathcal{S}\ni t\mapsto L_1(\underline{A}(t))$ is pluri-subharmonic and there exists $t_0$ such that $A(t_0)$ is projectively uniformly hyperbolic, so $L_1(t_0)>-\infty$. Therefore, 
%so as $L_1$ is pluri-subharmonic and $L_1\not\equiv -\infty$ we have that 
$L_1(\uA(t))>-\infty$ for $\Leb$-a.e. $t\in\mathcal{S}$.

Notice that $$\eta_t=\sum_{i\in\mathcal{A}_{sing}}\sum_{k\geq 0}\sum_{|{\omega}|=k}p_ip(\omega)\delta_{A^k_t(\omega)r_i(t)}$$ is the unique stationary measure and so, by the Furstenberg's formula we have that $L_1(A(t))=\int\psi_t d\eta_t$, where $\psi_t:\mathbb{P}^1\rightarrow\mathbb{R}$ is given by $\psi_t(\hat{v})=\sum_{j\in\mathcal{A}}p_j\log\norm{A_j(t)v}$.

By Theorem \ref{Uniform Ergodicity}, $$\norm{Q^n_t(\varphi)- \int \varphi \ d\eta_t}_\infty\leq 2(1-q)^n\norm{\varphi}_\infty,$$ $\forall\varphi\in C^0(\Pp^1) \ \forall n\geq 0$. Then we have a LDT for every $\varphi\in C^0(\Pp^1)$, i.e., $\forall v\in \Pp^1$ and $\forall n\geq 1$ $$\mathbb{P}_{\hat{v}}\bigg[\abs{\frac{1}{n}S_n\varphi-\int\varphi d\eta_t}>\epsilon \bigg]\leq 8e^{-c(\epsilon)n},$$ where $c(\epsilon)=c\epsilon^2\norm{\varphi}^{-2}_\infty$ (see Cai-Duarte-Klein 2022).



\begin{lemma}\label{L2}
$$\int_{\Lambda}\int_{\Pp^1}\psi^2_t d\eta_t dt < \infty$$ (and hence $\psi_t\in L^2(\eta_t)$ for a.e $t\in\Lambda$).
\end{lemma}

\begin{proof}
\begin{align*}
\int_{\Lambda}\int_{\Pp^1}\psi^2_t d\eta_t dt &\leq \int_\Lambda \sum_{i\in\mathcal{A}_{sing}}\sum_{k=0}^{\infty}\sum_{|\omega|=k}p_ip(\omega)\sum_{j\in\mathcal{A}}p_i\bigg(\log\frac{\norm{A_j(t)A^k_t(\omega)r_i(t)}}{\norm{A^k_t(\omega)r_i(t)}}\bigg)^2 \ dt\\
&\leq 2 \sum_{i\in\mathcal{A}_{sing}}\sum_{k=0}^{\infty}\sum_{|\omega|=k}\sum_{j\in\mathcal{A}}p_ip(\omega)p_j\int_\Lambda\bigg(\log^2(\norm{A_j(t)A^k_t(\omega)r_i(t)}\\
&+\log^2(\norm{A^k_t(\omega)r_i(t)}\bigg)dt
\end{align*}

Notice now that the function $\mathcal{S}\ni t\mapsto \log\norm{A_j(t)A^k_t(\omega)r_i(t)}$ is pluri-subharmonic, $\log\norm{A_j(t)A^k_j(\omega)r_i(t)}\lesssim k \ \forall t\in\mathcal{S}$ and $\log\norm{A_j(t_0)A^k_{t_0}(\omega)r_i(t_0)}\gtrsim -k$. So (by Cartan and Riesz (needs details)) we have that $$\int_\Lambda \log^2\norm{A_j(t)A^k_t(\omega)r_i(t)} dt\lesssim k^4.$$

Hence, as $\sum_{k=0}^{\infty}\sum_{|\omega|=k} p(\omega)=\sum_{k=0}^{\infty}(1-q)^k$, $$\int_{\Lambda}\int_{\Pp^1}\psi^2_t d\eta_t dt\lesssim \sum_{k=0}^\infty k^4(1-q)^k<\infty,$$ proving the lemma.

\end{proof}

\begin{remark}
Let $N\in\mathbb{N}$ and $B_N=\{(t,\hat{v})\in\Lambda\times\Pp^1: \psi_t(\hat{v})<-N\}$. Let ${\Tilde{\eta}}_t=\int \eta_t dt \in \Prob(\Lambda\times\Pp^1).$ Then by Lemma \ref{absl},
\begin{align*}
&\Tilde{\eta}(B_N)=\int_\Lambda \int_{\Pp^1} 1_{B_N}(t,\hat{v}) d\eta_t(\hat{v})dt\leq \\
&\leq\sum_{i\in\mathcal{A}_{sing}}\sum_{k=0}^{\infty}\sum_{|\omega|=k}p_ip(\omega)\int_\Lambda 1_{B_N}(t,A^k_t(\omega)r_i(t))dt\\
&\leq 
 e^{-N}.
\end{align*}
\end{remark}

\begin{remark} Note that by the H\"older inequality and Lemma ~\ref{L2} we have
$${\int\int}_{B_N}\abs{\psi_t}d\Tilde{\eta}\leq {\bigg(\int_\Lambda\int_{\Pp^1}{\abs{\psi_t}}^2 d\eta_t dt\bigg)}^{1/2}{\Tilde{\eta}(B_N)}^{1/2}\lesssim e^{-N/2}.$$
\end{remark}

Continuing with the proof of the Theorem, let $\psi_{t,N}(\hat{v})=\max\{\psi_t(\hat{v}),-N\}, \ N\in\mathbb{N}$. Notice that $\psi_{t,N}$ is continuous in $\hat{v}$ for every $t\in\Lambda$.
 

Now we have strong mixing for continuous abservable and so we have large deviations for $\psi_{t,N}$, meaning that 
$$\mathbb{P}_{\hat{v}}\left[\left|\frac{1}{n}S_n\psi_{t,N}-\int \psi_{t,N} d\eta_t\right|>\epsilon\right]<e^{-c(\epsilon)nN^{-2}}, \ \forall\hat{v}\in\Pp^1$$

Note that $$\abs{\frac{1}{n}S_n\psi_t - \int \psi_t d\eta_t}\leq
\abs{\frac{1}{n}S_n\psi_{t,N} - \int \psi_{t,N} d\eta_t} + \frac{1}{n}\abs{S_n(\psi_t-\psi_{t,N})} + \int\abs{\psi_t-\psi_{t,N}}d\eta_t.$$

Define $\mathcal{E}_N(t,\hat{v})=\frac{1}{n}\abs{S_n(\psi_{t,N}-\psi_t)} + \int \abs{\psi_{t,N}-\psi_t} d\eta_t$ and the events $$E_n(t,\hat{v},\epsilon):=\{\omega : \abs{\frac{1}{n}S_n\psi_t-\int\psi_t \ d\eta_t}>\epsilon\}$$ and $$\Delta_{n}(t,\hat{v},\epsilon,N):=\{\omega : \abs{\frac{1}{n}S_n\psi_{t,N}-\int \psi_{t,N} \ d\eta_t}\geq\epsilon\}.$$
We have that $$\int_{\Pp^1}\int_\Lambda \mathcal{E}_N(t,\hat{v})d\Tilde{\eta}\lesssim e^{-N/2}$$ and hence, if we define $$R_N:=\left\{(t,\hat{v}):\mathcal{E}_N(t,\hat{v})>e^{-N/4}\right\},$$ then by Markov's inequality, $\Tilde{\eta}(R_N)<e^{-N/4}$. Now, fix $\epsilon>0$. For $N$ large we have that $e^{-N/4}<\epsilon/2$ and so, if $(t,\hat{v})\notin R_N$, we have that $\mathcal{E}_N(t,\hat{v})\leq e^{-N/4}<\epsilon/2$. Furthermore $E_n(t,v,\epsilon)\subset\Delta_n(t,\hat{v},\epsilon/2,N)$, implying that $$\mathbb{P}_{\hat{v}}\left[E_n(t,\hat{v},\epsilon)\right]<e^{-c(\epsilon)nN^{-2}}, \ when \ (t,\hat{v})\notin R_N,$$ i.e., $$\mathbb{P}_{\hat{v}}\left[\left|\frac{1}{n}\log\norm{A^n_t v}-L_1(A_t)\right|>\epsilon\right]<e^{-c(\epsilon)nN^{-2}},$$ for some $\hat{v}$ such that $(t,\hat{v})\notin R_N$.\\
\\
As it is enough to prove the lower LDT,

\begin{equation}
\begin{aligned}
&\int \mathbb{P}\left[ \frac{1}{n}\log\norm{A^n_t}<L_1(A_t)-\epsilon \right] dt = \\
&\int \int \mathbb{P}_{\hat{v}}\left[\frac{1}{n}\log\norm{A^n_t}<L_1(A_t)-\epsilon \right] d{\eta}_t (\hat{v}) dt\\
&\leq \int \int \mathbb{P}_{\hat{v}}\left[\frac{1}{n}\log\norm{A^n_tv}<L_1(A_t)-\epsilon \right] d{\eta}_t (\hat{v}) dt\\
&\leq e^{-c\epsilon^2nN^{-2}} + e^{-N/4} \leq e^{-c\epsilon^2n^{1/3}},
\end{aligned}
\end{equation}
where we used $N=n^{1/3}$ for the latter inequality.

Hence, $$Leb\left(\left\{t: \mathbb{P}\left[ \frac{1}{n}\log\norm{A^n_t}-L_1(A_t)>e^{-{\epsilon}^2 n^{1/3}/2} \right]\right\}\right)<e^{-{\epsilon}^2 n^{1/3}/2}.$$
Let now $$B_n:=\left\{t: \mathbb{P}\left[ \frac{1}{n}\log\norm{A^n_t}-L_1(A_t)>e^{-{\epsilon}^2 n^{1/3}/2} \right]\right\}.$$ We have that $$\sum_{n=0}^{\infty}Leb(B_n)<\infty,$$ so by Borel Cantelli $\forall t \ \exists k_0$ s.t. $t\notin B^*_{k_0}$ where $$B^*_k:=\bigcup_{n=k}^{\infty}B_n,$$ then the LDT holds $\forall n\geq k$. Notice that the LDT estimates that we got are not uniform. In fact, if they were then $L_1$ would be H\"older continuous by the Abstract continuity theorem (see \cite{DK-book}).

\end{proof}
  
} 

==> statements.tex <==












==> stationary.tex <==

\medskip

In this section we establish  formulas for the stationary measure and the Lyapunov exponent of   a random linear cocycle $F \colon X\times \R^2\to X\times \R^2$ with rank $1$ determined by the data $(P, q,\uA)$
where $\uA :=(A_i)_{i\in\mathscr{A}} \in  \Mat_2(\R)^k$.
In the Bernoulli case, if we consider the $\Ascr$-valued Markov chain $\{\xi_n\}_n$ determined by $(P,q)$ then the sequence of return times to $\Asing$ forms a discrete time renewal process
~\cite[Definition 2.1]{Barbu2008}. Note that at these times, when $\xi_n=i\in \Asing$,  the $\uA$-induced  projective action  is reset 
to the range of $A_i$. This simple observation lies at the heart of all the explicit formulas presented below. Since in the Markov case the reduction to the setting of~\cite{Barbu2008} is less evident, the results of this section will be  presented for this case. The Bernoulli case can be treated similarly, but in a much more straightforward way; moreover, all relevant quantities have much simpler expressions.

Let $L^\infty(\Ascr\times\Pp^1)$ be the Banach space of bounded and measurable functions $\varphi \colon \Ascr\times\Pp^1\to\R$ endowed with the usual sup norm, denoted by $\norm{\cdot}_\infty$. Recall that the projective action of a nonzero matrix $A\in\Mat_2(\R)$ is given by $\hat A \hat v = \widehat{A v}$ if $A$ is invertible and by $\hat A \hat v=\hat r$, where $r=\Range (A)$ otherwise.

For the rank $1$ random cocycle  $\uA = (A_i)_{i\in\Ascr}\in\Mat_2(\R)^\Ascr$ we will use the notations $r_i$ and $k_i$ to represent, respectively, the range and the kernel of $A_i$, as well as, when convenient, a unit vector belonging to these one-dimensional subspaces. 

\newcommand{\Qinv}{\Qop_{\rm inv}}
\newcommand{\Qsing}{\Qop_{\rm sing}}


The cocycle $(P, q, \uA)$ determines the operator $\Qop \colon L^\infty(\Ascr\times\Pp^1)\to L^\infty(\Ascr\times\Pp^1)$
defined by
\begin{align*}
 (\Qop \varphi)(j,\hat v) &:= \sum_{ i\in\Ascr}  \varphi(i,\hat A_i\, \hat v)\, p_{ij} \\
& = \sum_{ i\in\Ainv}   \varphi(i, \hat A_i\, \hat v)\,p_{ij}  +  \sum_{ i\in\Asing} \varphi(i, \hat r_i)\,p_{ij} .
\end{align*}
Moreover, we write $\Qop = \Qinv + \Qsing$, where the operators $\Qinv$ and $\Qsing$ are given respectively by the two terms above. 

The operator $\Qop$ is clearly linear, positive and it takes the constant function $\ind$ to itself; in other words, it is a {\em Markov operator}. Let us recall the concept of stationary measure for such an operator.

\begin{definition}
A measure $\eta \in \Prob (\Ascr \times \Pp^1)$ is $\Qop$-stationary if for all observables $\varphi \in  L^\infty(\Ascr\times\Pp^1)$,
$$\int \Qop \varphi \, d \eta = \int \varphi \, d \eta .$$
In this case we also call $\eta$ stationary relative to the cocycle $(\uA, P, q)$.
\end{definition}

By general principles, a stationary measure always exists. In our setting it will be shown to be unique. 

Let $\pi \colon \Ascr\times \Pp^1\to  \Ascr$ denote the canonical projection in the first coordinate. If $\eta \in \Prob (\Ascr \times \Pp^1)$ is $\Qop$-stationary then its push-forward measure via $\pi$ is the $P$-stationary measure $q$ on $\Ascr$, that is, $\pi_\ast\eta=q$.

Indeed, the left stochastic matrix $P$ induces the Markov operator $u \mapsto u \, P$ on $L^\infty (\Ascr) \simeq \R^k$. For a (column) vector $q'$, $P q' = q'$ if and only if $u P q' = u q'$ for every (row) vector $u \in \R^k$, so $q'$ is $P$-stationary if and only if it is stationary relative to its corresponding Markov operator. Moreover, given any $u \in L^\infty (\Ascr)$ and using that $\eta$ is $\Qop$-stationary with the observable $\varphi := u \circ \pi$ it follows immediately that 
$$\int u P \, d (\pi_\ast\eta) = \int u \, d (\pi_\ast\eta) ,$$
showing that $\pi_\ast\eta$ is $P$-stationary. But since $P$ is primitive, it has a unique stationary probability vector, so $\pi_\ast\eta = q$.

\smallskip  

Since $\eta$ projects down via $\pi$ to $q$, we can consider 
its disintegration $\{\eta_i\}_{i\in\Ascr} \subset \Prob (\Pp^1)$, which is characterized by 
$$\int_{\Ascr\times\Pp^1}  \varphi (i, \hat v) \, d \eta (i, \hat v) = \sum_{i\in\Ascr} \, q_i \, \int_{\Pp^1} \varphi (i, \hat v) \, d \eta_i (\hat v) \quad \forall \varphi \in L^\infty(\Ascr\times\Pp^1) \, .$$

Then
\begin{equation*}
\eta=\sum_{i\in\Ascr} q_i\, \delta_i\times\eta_i \quad \text{and} \quad \eta_i (E) = \frac{1}{q_i} \, \eta (\{i\} \times E) \,\, \forall i\in \Ascr, E\subset \Pp^1 \text{ Borel} .
\end{equation*}

Moreover, the disintegration of a stationary measure satisfies the following properties (see also~\cite{Viana-M} for the setting of invertible Markov cocycles).  

\begin{lemma}\label{statmeas}
Let $\eta$ be a stationary measure for the rank $1$ random cocycle $(\uA, P, q)$ and let $\{\eta_i\}_{i\in\Ascr}$ be its disintegration over the projection $\pi$ (recall that $\pi_\ast \eta=q$).  Then
\begin{enumerate}
	\item $\eta_j(\{\hat k_j\})=0$ for all $j\in\Asing$,
	\item $\displaystyle  \eta_j=\frac{1}{q_j} \sum_{i \in\Ascr} q_i p_{j i} (\hat A_j)_\ast \eta_i \quad \text{ for all }\,  j\in\Ascr . $
\end{enumerate}	
\end{lemma}

\begin{proof}
Let $j\in\Asing$ and consider the observable $\ind_{\{(j, \hat k_j)\}} \in L^\infty(\Ascr\times\Pp^1)$. Then since $\eta$ is $\Qop$-stationary,
\begin{align*}
\eta_j(\{\hat k_j\}) &= \frac{1}{q_j} \, \int \ind_{\{(j, \hat k_j)\}} \, d \eta =  \frac{1}{q_j} \, \int \Qop \ind_{\{(j, \hat k_j)\}} (l, \hat v) \, d \eta (l, \hat v) \\
& =  \frac{1}{q_j} \, \int \left( \sum_{i\in\Ascr} \ind_{\{(j, \hat k_j)\}} (i, \hat A_i \hat v) \, p_{i l} \right)  d \eta (l, \hat v) =  \frac{1}{q_j} \, \int 0 \, d \eta = 0 .
\end{align*} 
The penultimate equality follows from the fact that  $j\in\Asing$, so that $\hat A_j \hat v = \hat r_j \neq \hat k_j$, since $\uA$ does not contain null words.

\medskip

To prove the second statement let $j\in\Ascr$ and given any $\varphi\in L^\infty(\Pp^1)$ define its extension $\varphi_j \in L^\infty(\Ascr\times\Pp^1)$ by
$$\varphi_j  (i, \hat v):=\begin{cases}
\varphi (\hat v) & \text{ if }  i=j\\
0 & \text{otherwise} .
\end{cases} $$
The characterization of the disintegration applied to $\varphi_j$ immediately implies that
$$\int \varphi \, d \eta_j = \frac{1}{q_j} \, \int \varphi_j \, d \eta .$$
Moreover, since $\eta$ is $\Qop$-stationary,
\begin{align*}
 \int \varphi_j \, d \eta &=  \int \Qop \varphi_j (l, \hat v) \, d \eta (l, \hat v) =
 \int \left( \sum_{i\in\Ascr} \varphi_j (i, \hat A_i \hat v) \, p_{i l} \right) \, d \eta (l, \hat v)\\
 &= \int \left( \varphi (\hat A_j \hat v)  \, p_{j l} \right) \, d \eta (l, \hat v) =
 \int \sum_{i\in\Ascr} q_i \, \varphi (\hat A_j \hat v) \, p_{j i} \, d \eta_i (\hat v)  \\
 &= \int \sum_{i\in\Ascr} q_i \, p_{j i} \, \varphi (\hat v) \,  d (\hat A_j)_\ast \eta_i (\hat v)
\end{align*} 
which establishes the second identity since $\varphi$ is arbitrary. The penultimate equality above follows from the fact that $\eta=\sum_{i\in\Ascr} q_i\, \delta_i\times\eta_i$.
\end{proof}

\smallskip

Given $n\ge 1$, $s \in \Asing$ and $l \in\Ascr$, let $\Bscr_{n}(s,l)$ denote the set of admissible words $\uom=(\omega_0, \ldots, \omega_{n})$
of length $n+1$ such that $\omega_0=s$, $\omega_{n}=l$  and 
$\omega_i\in \Ainv$ for all $i=1, \ldots, n-1$.
For such a word we write
$A^{n}(\uom):=A_{\omega_{n}}\, \ldots\, A_{\omega_2}\, A_{\omega_1}$  as in the previous section, and also put
  $p (\uom):=p_{\omega_n\,\omega_{n-1}} \, \cdots \, p_{\omega_1\,\omega_{0}}$. 
  
With these notations, we have the following explicit formula for a (or, a-posteriori, {\em the}) $\Qop$-stationary measure. 

\medskip

\begin{proposition}
\label{prop stationary measure}
Let $\eta=\displaystyle\sum_{j \in \Ascr}q_j\delta_j \times \eta_j$
where for all $j\in\Ascr$,

$$
\eta_j := \frac{1}{q_j} \sum_{s \in \Asing}q_s \sum_{n=1}^\infty
\sum_{\uomega \in \Bscr_{n}(s, j)}  p(\uomega)\delta_{\hat A^n(\uomega) \hat r_s}.
$$
Then $\eta$ is a $(P, q, \uA)$-stationary probability measure on $\Ascr\times\Pp^1$.
\end{proposition}

\begin{proof} We first show that for all $j\in\Ascr$,
\begin{equation}
\label{q formula}
	\sum_{s \in \Asing}q_s \sum_{n=1}^\infty
	\sum_{\uomega \in \Bscr_{n}(s,j)}  p(\uomega)=q_j .
\end{equation}
This will then imply that $\eta_j$ is a probability measure on $\Pp^1$ for all $j\in\Ascr$, hence $\eta$ is a probability measure on $\Ascr\times\Pp^1$.

Indeed, given $j\in\Ascr$, consider the cylinder $[0; j]$ determined by the word $(j)$, so $\mu ([0; j]) = q_j$. This cylinder is partitioned, modulo a zero  measure set (mod $0$), into cylinders $[-n; s \uom' j]$, determined by admissible words $(s, \uom', j)$ where $s\in\Asing$ and $\uom' = (\om_1, \cdots, \om_{n-1})$ with $\om_i \in \Ainv$ for all $1\le i \le n-1$, $n\ge 0$ (when $n=1$,   the word $(s, \uom', j)$ is simply $(s, j)$).  In other words,
$$[0; j] = \bigsqcup_{s\in\Asing} \, \bigsqcup_{n=1}^\infty \, \bigsqcup_{\om=(s, \uom', j) \in \Bscr_n (s, j)} \, [-n; s \uom' j] \, (\mod 0) . $$

The cylinders $[-n; s \uom' j]$ are mutually disjoint because $s\in\Asing$ and $\om_i\in\Ainv$ for all $i$. Modulo a zero measure set, their union is $[0; j]$ since, by the mixing of the Markov shift determined by $(P, q)$, almost every admissible infinite word starting with the symbol $j$ contains in its past a symbol $s\in\Asing$. Moreover, 
$\mu ( [-n; s \uom' j] ) = q_s \, p (s, \om', j)$ which establishes the identity~\eqref{q formula}.

It remains to verify that $\eta=\sum_{j \in \Ascr}q_j\delta_j \times \eta_j$ is $\Qop$-stationary, that is, 
$\int \Qop \varphi \, d \eta = \int \varphi \, d \eta$ for all $\varphi \in L^\infty (\Ascr \times \Pp^1)$. 


\smallskip


Firstly note that if $j\in\Asing$ then $\eta_j = \delta_{\hat r_j}$. 
Indeed, for all $n\ge 1$, $s\in\Asing$, $\uom \in \Bscr_n (s, j)$ we have
$\hat A^n (\uom) \hat r_s = \hat A_j \cdots \hat A_{\om_1} \hat r_s = \hat r_j$, 
so using the identity~\eqref{q formula},
\begin{align*}
\eta_j &= \frac{1}{q_j} \sum_{s \in \Asing}q_s \sum_{n=1}^\infty
\sum_{\uomega \in \Bscr_{n}(s, j)}  p(\uomega)\delta_{\hat A^n(\uomega) \hat r_s} \\
& =
\frac{1}{q_j} \Big(  \sum_{s \in \Asing}q _s \sum_{n=1}^\infty
\sum_{\uomega \in \Bscr_{n}(s, j)}  p(\uomega) \Big) \, \delta_{\hat r_j} = \delta_{\hat r_j} .
\end{align*}

Secondly, for any observable $\varphi \in L^\infty (\Ascr \times \Pp^1)$, we write
\begin{align*}
\int \varphi \, d \eta = \sum_{j\in\Ascr} q_j \, \int \varphi (j, \hat v) \, d \eta_j (\hat v) = \Sinv (\varphi) + \Ssing (\varphi)
\end{align*}
where
\begin{align*}
\Sinv (\varphi) &:= \sum_{j\in\Ainv} q_j \, \int \varphi (j, \hat v) \, d \eta_j (\hat v) \\
&= \sum_{j\in\Ainv} \, \sum_{s\in\Asing} q_s \, \sum_{n=1}^\infty \sum_{\uom\in\Bscr_n (s, j)} p (\uom) \, \varphi (j, \hat A^n(\uomega) \hat r_s)
\end{align*}
and
\begin{align*}
\Ssing (\varphi) &:= \sum_{j\in\Asing} q_j \, \int \varphi (j, \hat v) \, d \eta_j (\hat v) = \sum_{j\in\Asing} q_j \, \varphi (j, \hat r_j) \, .
\end{align*}

Recall that $\Qop \varphi = \Qinv \varphi + \Qsing \varphi$, where
\begin{align*}
\Qinv \varphi (j, \hat v) &= \sum_{ i\in\Ainv}  p_{ij} \,   \varphi(i, \hat A_i\, \hat v)\\
\Qsing \varphi (j, \hat v) &= \sum_{ i\in\Asing} p_{ij} \, \varphi(i, \hat r_i) \, .
\end{align*}

Then
\begin{align*}
\int \Qop \varphi \, d \eta &= \Sinv (\Qop \varphi) + \Ssing (\Qop \varphi) \\
&= \Sinv (\Qinv \varphi) + \Sinv (\Qsing \varphi) + \Ssing (\Qinv \varphi) + \Ssing (\Qsing \varphi) \, .
\end{align*}

We evaluate each of the four terms above separately.
\begin{align*}
\Sinv (\Qinv \varphi) &=  \sum_{j\in\Ainv} \, \sum_{i\in\Ainv} \,  \sum_{s\in\Asing} q_s \, \sum_{n=1}^\infty \sum_{\uom\in\Bscr_n (s, j)} p (\uom) \, p_{i j} \, \varphi (i, \hat A_i \hat A^n(\uomega) \hat r_s)\\
&=  \sum_{i\in\Ainv} \, \sum_{s\in\Asing} q_s \, \sum_{n=1}^\infty \sum_{\uom'\in\Bscr_{n+1} (s, i)} p (\uom') \, \varphi (i, \hat A^n(\uomega') \hat r_s)\\
&=  \sum_{i\in\Ainv} \, \sum_{s\in\Asing} q_s \, \sum_{n=2}^\infty \sum_{\uom\in\Bscr_{n} (s, i)} p (\uom) \, \varphi (i, \hat A^n(\uomega) \hat r_s) \, .
\end{align*}
The first line turned into the second by adding the letter $i$ to the end of the word $\uom\in\Bscr_n (s, j)$ with $j\in\Ainv$, so that $\uom' := (\uom, i) \in \Bscr_{n+1} (s, i)$; note that $p (\uom') = p_{i j} \, p(\uom)$. 

Similarly,
\begin{align*}
\Sinv (\Qsing \varphi) &=  \sum_{j\in\Ainv} \, \sum_{i\in\Asing} \,  \sum_{s\in\Asing} q_s \, \sum_{n=1}^\infty \sum_{\uom\in\Bscr_n (s, j)} p (\uom) \, p_{i j} \, \varphi (i, \hat r_i)\\
&=  \sum_{i\in\Asing} \, \sum_{s\in\Asing} q_s \, \sum_{n=1}^\infty \sum_{\uom'\in\Bscr_{n+1} (s, i)} p (\uom') \, \varphi (i,  \hat r_i)\\
&=  \sum_{i\in\Asing} \, \sum_{s\in\Asing} q_s \, \sum_{n=2}^\infty \sum_{\uom\in\Bscr_{n} (s, i)} p (\uom) \, \varphi (i,  \hat r_i) \, .
\end{align*}

Then
\begin{align*}
\Ssing (\Qinv \varphi) &=  \sum_{j\in\Asing} q_j \sum_{i\in\Ainv} p_{i j} \, \varphi (i,  \hat A_i \hat r_j)\\
&=  \sum_{i\in\Ainv} \, \sum_{s\in\Asing} q_s \, \sum_{\uom\in\Bscr_{1} (s, i)} p (\uom) \, \varphi (i, \hat A^1 (\uom)  \hat r_s)
\end{align*}
where in passing from the second to the last line we changed the index $j$ for $s$ and used the fact that $(s, i)$ is the only word $\uom\in\Bscr_1 (s, i)$ and in this case $p(\uom)=p_{i s}$ and $A^1 (\uom)=A_i$.

Finally,
\begin{align*}
\Ssing (\Qsing \varphi) &=  \sum_{j\in\Asing} q_j \sum_{i\in\Asing} p_{i j} \, \varphi (i,  \hat r_i)\\
&=  \sum_{i\in\Asing} \, \sum_{s\in\Asing} q_s \, \sum_{\uom\in\Bscr_{1} (s, i)} p (\uom) \, \varphi (i,  \hat r_i) \, .
\end{align*}

Note that 
$\Sinv (\Qinv \varphi) + \Ssing (\Qinv \varphi) = \Sinv (\varphi)$
and using again~\eqref{q formula},
\begin{align*}
\Sinv (\Qsing \varphi) + \Ssing (\Qsing \varphi) &=  \sum_{i\in\Asing} \Big(\sum_{s\in\Asing} q_s  \sum_{n=1}^\infty \sum_{\uom\in\Bscr_{n} (s, i)} p (\uom)\Big)  \varphi (i,  \hat r_i) \\
&=  \sum_{i\in\Asing} q_i \,  \varphi (i,  \hat r_i) = \Ssing (\varphi) ,
\end{align*}
which concludes the proof.
\end{proof}




\begin{theorem} \label{Uniform Ergodicity} If the cocycle $(P, q,\uA)$ has rank one, then $\Qop$ is uniformly ergodic, i.e. there exist constants $C<\infty$ and $a>0$ such that
$$  \norm{  \Qop^n\varphi - \int\varphi\, d\eta }_\infty \leq C\, e^{-a\,n}\,\norm{\varphi}_\infty $$
for all $n\in\N$ and  
$\varphi\in L^\infty(\Ascr\times\Pp^1)$, where $\eta$ is any $\Qop$-stationary measure.
\end{theorem}

\begin{proof} Note that $L^\infty (\Ascr) \simeq \R^k$, seen as the subspace of observables $\varphi$ that do not depend on the projective variable, is invariant under the Markov operator $\Qop$; when restricted to this subspace, $\Qop$ becomes the operator $u \mapsto u \, P$ induced by the left stochastic matrix $P$. Recall also that $\eta$ projects down to $q$, the stationary probability vector of $P$. Since $P$ is primitive, for some constants $C<\infty$ and $\sigma \in (0, 1)$ (these constants may change a few times throughout the argument) 
\begin{equation}\label{eq 999}
\norm{u \, P^n - u \cdot q}_\infty \le C \sigma^n \, \norm{u}_\infty
\end{equation}
for all $n\in\N$ and $u \in \R^k \simeq L^\infty (\Ascr)$.

We show that for all $n\in\N$ there is a linear operator $T_n \colon L^\infty(\Ascr\times\Pp^1) \to L^\infty(\Ascr)$ such that for all $\varphi\in L^\infty(\Ascr\times\Pp^1)$,
\begin{equation}\label{eq1000}
\Qop^n \varphi = \Qinv^n \varphi + T_n \varphi .
\end{equation}
In other words, $\Qop^n \varphi - \Qinv^n \varphi$ does not depend on the projective variable. 

Indeed, when $n=1$, $\Qop \varphi = \Qinv \varphi + \Qsing \varphi$, where $\Qsing \varphi (j, \hat v) = \sum_{i\in\Asing} \varphi (i, \hat r_i) \, p_{i j} =: T_1 \varphi (j)$ does not depend on $\hat v$. By induction, if we assume that for all observables $\varphi$ we can write $\Qop^n \varphi = \Qinv^n \varphi + T_n \varphi$ with $T_n \varphi$ not depending on the projective variable, then
\begin{align*}
\Qop^{n+1} \varphi &= \Qop (\Qop^n \varphi) = \Qop (\Qinv^n \varphi + T_n \varphi) 
=  \Qop (\Qinv^n \varphi) + \Qop (T_n \varphi) \\
&= \Qinv (\Qinv^n \varphi) + \Qsing (\Qinv^n \varphi) +  (T_n \varphi) \, P
= \Qinv^{n+1} \varphi  + T_{n+1} \varphi ,
\end{align*}
where 
\begin{equation}\label{eq1002}
T_{n+1} \varphi :=  \Qsing (\Qinv^n \varphi) +  (T_n \varphi) \, 
\end{equation}
does not depend on the projective variable, thus establishing the claim~\eqref{eq1000}.

\smallskip

We show that $\Qinv^n$ eventually contracts, so $\Qinv^n \varphi$ converges exponentially fast to $0$, while  $T_n \varphi$ converges exponentially fast to a constant (in the sup norm), which immediately imply the conclusion of the theorem. 

\smallskip

Since the stochastic matrix $P$ is primitive, there is $N\ge1$ such that $P^N_{i j} > 0$ for all $i, j \in \Ascr$. In particular, since $P^N$ is also stochastic,
$$\sigma_0 := \max_{j\in\Ascr} \, \sum_{i\in\Ainv} \, P^N_{i j} < 1 .$$

We show that $\Qinv^N$ is a contraction on $L^\infty(\Ascr\times\Pp^1)$. Indeed, given any observable $\varphi$ and $(j, \hat v) \in \Ascr \times \Pp^1$, clearly
$$\Qinv^N \varphi (j, \hat v) = \sum_{i\in\Ainv} \, \sum_{\uom\in\Bscr_N (j, i)} \varphi (i, A^N (\uom) \hat v) \, p (\uom) \, .$$
Then
\begin{align*}
\norm{\Qinv^N \varphi}_\infty &\le \norm{\varphi}_\infty \, \max_{j\in\Ascr} \, \sum_{i\in\Ainv} \, \sum_{\uom\in\Bscr_N (j, i)} p (\uom) \\
&= \norm{\varphi}_\infty \, \max_{j\in\Ascr} \, \sum_{i\in\Ainv} \, \sum_{\uom'\in\Ainv^{N-1}} p ( j \uom' i)\\
&\le \norm{\varphi}_\infty \, \max_{j\in\Ascr} \, \sum_{i\in\Ainv} \, \sum_{\uom'\in\Ascr^{N-1}} p ( j \uom' i)\\
&=  \norm{\varphi}_\infty \, \max_{j\in\Ascr} \, \sum_{i\in\Ainv} \, P^N_{i j} = \sigma_0 \,  \norm{\varphi}_\infty \, .
\end{align*}

Given any integer $n$, we write $n = m N + r$ with $0\le r < N$ and use the fact that the operator norm of $\Qinv$ is equal to $1$ to then conclude that for some $C<\infty$ and $\sigma \in (0, 1)$,
\begin{equation}\label{eq1001}
\norm{\Qinv^n \varphi}_\infty \le C \sigma^n \, \norm{\varphi}_\infty
\end{equation}
for all $n\in\N$ and $\varphi\in L^\infty(\Ascr\times\Pp^1)$.


\smallskip

From~\eqref{eq1002} and~\eqref{eq1001} we get that for all $n\in\N$,
$$\norm{ T_{n+1} \varphi - (T_n \varphi) \, P}_\infty = \norm{ \Qsing (\Qinv^n \varphi) }_\infty \le 
\norm{\Qinv^n \varphi}_\infty \le C \sigma^n \, \norm{\varphi}_\infty .$$

Then
\begin{align*}
\norm{T_{n+2} \varphi  - (T_n \varphi) \, P^2}_\infty &\le \norm{ T_{n+2} \varphi - (T_{n+1} \varphi) \, P}_\infty +
\norm{ (T_{n+1} \varphi  - (T_{n} \varphi) P) \, P}_\infty \\
&\le C (\sigma^n + \sigma^{n+1})\, \norm{\varphi}_\infty ,
\end{align*}
so proceeding inductively, for all $n, k \in \N$, 
$$\norm{ T_{n+k} \varphi - (T_n \varphi) \, P^k}_\infty \le C' \sigma^n \, \norm{\varphi}_\infty .$$

In particular,
\begin{equation}\label{eq1005}
\norm{ T_{2 n} \varphi - (T_n \varphi) \, P^n}_\infty \le C' \sigma^n \, \norm{\varphi}_\infty .
\end{equation}

By~\eqref{eq 999},
\begin{equation}\label{eq1006}
\norm{(T_n \varphi) \, P^n - (T_n \varphi) \cdot q}_\infty \le C \sigma^n \, \norm{(T_n \varphi)}_\infty \le 2 C \sigma^n \, \norm{\varphi}_\infty \, .
\end{equation}

We have $\Qop^n \varphi = \Qinv^n \varphi  + T_n \varphi $. Since the measure $\eta$ is $\Qop$-stationary and it projects down to $q$, it follows that
\begin{align}
\abs{ \int \varphi d \eta -  (T_n \varphi) \cdot q} &= \abs{ \int \Qop^n \varphi \, d \eta -   \int T_n \varphi \, d\eta } \notag\\
& = \abs{ \int \Qinv^n \varphi \, d \eta} \le \norm{\Qinv^n \varphi}_\infty \le C \sigma^n \, \norm{\varphi}_\infty . \label{eq1007}
\end{align}

Combining~\eqref{eq1005},~\eqref{eq1006} and~\eqref{eq1007}, we conclude that
\begin{equation*}\label{eq1010}
\norm{ T_{2 n} \varphi -  \int \varphi d \eta}_\infty \le C'' \sigma^n \, \norm{\varphi}_\infty ,
\end{equation*}
which, together with~\eqref{eq1001} establishes our result (after choosing the constants $C, a$ appropriately).
\end{proof}

\begin{corollary}
If the cocycle $(P, q,\uA)$ has rank one, then it admits a unique stationary measure.
\end{corollary}

\begin{proof}
If $\eta_1$ and $\eta_2$ are $\Qop$-stationary, then Theorem~\ref{Uniform Ergodicity} above applies to each of them, so 
for any $\varphi\in L^\infty(\Ascr\times\Pp^1)$, $\Qop^n \varphi$ converges uniformly to $\int \varphi \, d \eta_1$ and to $\int \varphi \, d \eta_2$. Thus $\int \varphi \, d \eta_1 = \int \varphi \, d \eta_2$ for all observables $\varphi$, showing that $\eta_1 = \eta_2$.
\end{proof}



\begin{lemma} \label{prodNorm}
Given rank one matrices 
	$B_1, B_2, \dots , B_n$ and a unit vector $r_0$,  it follows that
$$
\norm{B_{n} \cdots B_{1}\, r} = \prod_{l=1}^n\norm{B_{l}\, r_{l-1}} \, ,
$$
where $ r_{l-1}$  is a unit vector in the range of $B_{l-1}$.
\end{lemma}

\begin{proof}
We write $B_1 r_0 = \la_1 r_1$, thus $\sabs{\la_1} = \norm{B_1 r_0}$. It follows that 
$B_2 B_1 r_0 = \la_1 B_2 r_1$ so 
$$\norm{B_2 B_1 r_0} = \sabs{\la_1} \norm{B_2 r_1} = \norm{B_2 r_1} \norm{B_1 r_0} \, .$$
From here,
$$
\norm{B_{n+1} B_n \big(B_{n-1} \cdots B_{1}\, r_0 \big) } = \norm{ B_{n+1} r_n} \norm{ B_n \big(B_{n-1} \cdots B_{1}\, r_0 }$$ 
and the conclusion follows by induction.
\end{proof}



\begin{lemma} \label{propL1}
For a rank one Markov cocycle determined by $(P, q, \uA)$,
$$
L_1(\uA) = \sum _{i \in \Asing} \sum _{j \in \Asing} \sum _{n=1}^\infty \sum _{\uom\in \Bscr_{n}(i, j)} q_i \, p(\uom) \, \log \norm{A^n(\uom) r_i} \, .
$$
\end{lemma}

\begin{proof}
Consider the cylinders $C_i := [0; i]$ with $i \in \Asing$ and their union $C:= \bigcup_{i \in \Asing} C_i$, the set of all (bi-infinite) words with a singular symbol at the zeroth position. Then $q:= \mu(C) = \sum_{i\in \Asing} q_i$.

Moreover, let $\displaystyle C_{i, j}:= \bigcup_{n=1}^\infty \, \bigcup_{\uom\in \Bscr_{n}(i, j)} [0; \uom]$. By the mixing of the Markov shift, these sets give rise to the  following partitions modulo a zero measure set (mod $0$)
\begin{align*}
C_i &= \bigcup_{j \in \Asing}C_{i, j} =\bigcup_{j \in \Asing}\bigcup_{n=1}^\infty \, \bigcup_{\uom\in \Bscr_{n}(i, j)} [0; \uom] \;  \text{ and } \\
C & = \bigcup_{j \in \Asing}\bigcup_{i \in \Asing}C_{i, j} = \bigcup_{i \in \Asing}\bigcup_{j \in \Asing} \, \bigcup_{n=1}^\infty \, \bigcup_{\uom\in \Bscr_{n}(i, j)} [0; \uom] \, .
\end{align*}

Let $g \colon C \to C$ be the first return map to the cylinder $C$, given by $g(\omega)=\sigma^{\tau(\omega)}(\omega)$, where $\tau(\omega)=\min\{k \ge 1 \colon \sigma^k (\om) \in C \}$. The map $g$ preserves the induced measure $\bar \mu_C=\mu(C)^{-1}\, \mu|_C = \frac{1}{q} \, \mu|_C $.


We define the induced cocycle $F_C \colon C\times \R^2 \to C \times \R^2$, given by $F_C(\omega,v):=(g(\omega), \Ccal (\om) \,v)$, where $\Ccal (\om) := A^{\tau(\omega)}(\omega)$. 

By \cite[Proposition 4.18 and Exercise 4.8]{Viana2014} (it is easy to verify that these statements also hold for $\Mat_2 (\R)$-valued fiber maps) its Lyapunov exponent is related to that of the original cocycle $(P, q, \uA)$ via the expression $L_1(F_C)=\frac{1}{q} L_1(\uA)$; thus it is enough to compute $L_1(F_C)$. 

The induced cocycle $F_C$ leaves invariant the $1$-dimensional sub-bundle $X \ni \om \mapsto R(\omega):= \mathrm{Range}( A_{\omega_0})$.
Then using Oseledets' theorem, its first Lyapunov exponent is the rate of exponential growth of the fiber iterates of $F_C$ along this sub-bundle. Thus for $\mu$-a.e. $\om \in C$ and for a unit vector $r_0 \in R (\om) = \mathrm{Range}( A_{\omega_0})$,
\begin{equation}\label{eq 100}
L_1(F_C) = \lim_{n \to \infty} \frac{1}{n}\log \norm{\mathcal{C}^n(\omega) \, r_0}
= \lim_{n \to \infty} \frac{1}{n}\log \ \prod_{l=1}^{n} \norm{\Ccal (g^l\omega) \, r_0} \, .
\end{equation}


Given $\om \in C$, let $0 = k_1 < k_2 < \cdots $ denote all future entries to the singular part of the alphabet, that is, $k \in \N$ is such that $\om_k \in \Asing$ if and only if $k = k_l$ for some $l\in\N$. Then clearly $g^l (\om) = \sigma^{k_l} (\om)$ (whose zeroth entry is $\om_{k_l}$) and $\tau (g^l \om) = k_{l+1} - k_l$ for all $l\in\N$. Moreover, 
$$B_l := \Ccal (g^l\om) = A^{\tau (g^l \om)} (g^l \om) = A^{k_{l+1} - k_l} (\sigma^{k_l} \om)
= A_{\om_{k_{l+1}}} \cdots  A_{\om_{k_{l}+1}} \, ,$$
which is a rank one matrix whose range $r_l :=  \mathrm{Range} (B_l) = r_{\om_{k_{l+1}}} $.

By Lemma~\ref{prodNorm},
\begin{align}
\norm{\Ccal^n(\omega) \, r_0} &=  \norm{\prod_{l=n}^{1} \Ccal (g^l\omega) \, r_0} 
 =  \norm{\prod_{l=n}^{1} B_l \, r_0} =  \prod_{l=1}^n\norm{B_{l}\, r_{l-1}} \notag\\
& =  \prod_{l=1}^n \norm{ \Ccal (g^l \om) \, r_{\om_{k_{l}}} } \, . \label{eq 99}
\end{align}

Consider the observable $\varphi \colon C \to \R$, 
$$\varphi (\om) := \log \norm{\Ccal (\om) \, r_{\om_0} } = \log \norm{A^{\tau(\om)} (\om) \, r_{\om_0} } .$$
By~\eqref{eq 100},~\eqref{eq 99} and Birkhoff's ergodic theorem,
\begin{align*}
L_1(F_C) &=  \lim_{n \to \infty} \frac{1}{n} \sum_{l=1}^{n} \log \norm{ \Ccal (g^l \om) \, r_{\om_{k_{l}}} } 
=  \lim_{n \to \infty} \frac{1}{n} \sum_{l=1}^{n} \varphi (g^l \om) \\
&= \int_C  \varphi (\om) \, d \bar{\mu}|_C (\om)  = \frac{1}{q} \int_C \log \norm{\Ccal (\om) \, r_{\om_0} } \, d \mu (\om) \, .
\end{align*}

Note that on each given cylinder $[0; \uom]$ with $\uom\in \Bscr_{n}(i, j)$ for some $i, j \in \Asing$ and $n\ge 1$, the first return map $\tau$ is constant and equal to $n$, while the observable $\varphi$ is equal to
$\log \norm{A^n (\om)  \, r_{\om_0}} = \log \norm{A^n (\uom) \, r_i}$, thus it is constant. 
Moreover, the Markov measure of this cylinder is $\mu [0; \uom] = q_i \, p (\uom)$. Since these cylinders partition (mod $0$) the set $C$, we conclude that
$$\int_C \varphi (\om) \, d \mu (\om) = \sum_{i, j \in\Asing} \, \sum_{n=1}^\infty \, \sum_{\uom \in \Bscr_n (i, j)} q_i \, p (\uom)
\,   \log \norm{A^n (\uom) \, r_i} \, ,$$
which completes the proof of the lemma.
\end{proof}

Consider the following observable $\Psi \colon \Ascr\times \Proj \to [- \infty, \infty)$,
$$
\Psi (j, \hat v) = \sum_{i \in \Ascr} p_{i j}\, \log \frac{\norm{A_i\, v}}{\norm{v}} .
$$

\begin{theorem}[Furstenberg's Formula] \label{Furstenberg's Formula} 
If the cocycle $(P, q,\uA)$ has rank one then
$$
L_1(\uA) = \int \Psi \; d\eta .
$$
\end{theorem}



\begin{proof} 
Using the explicit formula of the stationary measure $\eta$ derived in Proposition~\ref{prop stationary measure},
\begin{align*}
\int  \Psi \ d\eta &= \sum_{l\in\Ascr}  \, \sum_{i\in \Ascr} p_{il}  \sum_{s\in \Asing}q_s\sum_{n=1}^{\infty}\sum_{\uom\in \Bscr_n (s, l)} p(\uomega)\log\frac{\norm{A_i\, A^n(\uomega)\,r_s}}{\norm{A^n(\uomega)\,r_s}} .
\end{align*}

For $\uom\in\Bscr_n (s, l)$ with $l\in\Asing$,  $\hat A^n(\uomega)\, \hat r_s = \hat A_l \cdots \hat A_{\om_1} \, \hat r_s = \hat r_l$. The expression above can then be split into
\begin{align*}
&\sum_{l\in\Asing} \sum_{i\in\Ascr}p_{il}\sum_{s\in \Asing}q_s\sum_{n=1}^{\infty}\sum_{\uomega\in\Bscr_n(s, l)} p(\uomega)\log\norm{A_i\,r_l}\\
&+ \sum_{l\in\Ainv}\sum_{i\in\Ascr}p_{il}\sum_{s\in \Asing}q_s\sum_{n=1}^{\infty}\sum_{\uomega\in\Bscr_n(s,l)} p(\uomega)\log\frac{\norm{A_i\, A^n(\uomega)\, r_s}}{\norm{A^n(\uomega)\,r_s}} .
\end{align*}

By~\eqref{q formula} we have $\sum_{s\in \Asing}q_s\sum_{n=1}^{\infty}\sum_{\uomega\in\Bscr_n(s, l)} p(\uomega) = q_l $ which, when used in the first term above, turns the last expressions into
\begin{align*}
&\sum_{l\in\Asing}\sum_{i\in\Ascr}p_{il}\,q_l\,\log\norm{A_i\,r_l}\\
&+\sum_{l\in\Ainv}\sum_{i\in\Ascr}p_{il}\sum_{s\in \Asing}q_s\sum_{n=1}^{\infty}\sum_{\uomega\in\Bscr_n(s, l)} p(\uomega)\log\norm{A_i\,A^n(\uomega)\,r_s}\\
&-\sum_{l\in\Ainv}\sum_{i\in\Ascr}p_{il}\sum_{s\in \Asing}q_s\sum_{n=1}^{\infty}\sum_{\uomega\in\Bscr_n(s, l)} p(\uomega)\log\norm{A^n(\uomega)\,r_s} \\
\\
&= \sum_{l\in\Asing}\sum_{i\in\Ascr}p_{il}\,q_l\,\log\norm{A_i\,r_l}\\
&+\sum_{i\in\Ascr}\sum_{s\in\Asing} q_s\sum_{n=2}^{\infty}\sum_{\uomega' \in \Bscr_n(s, i)}p(\uomega')\log\norm{A^n(\uomega')\, r_s} \\
&-\sum_{l\in\Ainv}\sum_{s\in \Asing}q_s\sum_{n=1}^{\infty}\sum_{\uomega\in\Bscr_n(s, l)} p(\uomega)\log\norm{A^n(\uomega)\,r_s} \, .
\end{align*}
The third line above turned into the sixth because $\sum_{i\in\Ascr} p_{il} = 1$. The second line turned into the fifth by adding the letter $i$ to the end of the word $\uom\in\Bscr_n (s, l)$ with $l\in\Ainv$, so that $\uom' := (\uom, i) \in \Bscr_{n+1} (s, i)$; note that $p (\uom') = p_{i l} \, p(\uom)$. 

The last two lines above cancel each other out partially (note the slight difference in the ranges of the index $n$ and the fact that the final letter in the words appearing in the penultimate term ranges over the whole alphabet, while in the ultimate  term it ranges only over the invertible part). The whole expression is then equal to
 \begin{align*}
& \sum_{l\in\Asing}\sum_{i\in\Ascr}p_{il}\,q_l\,\log\norm{A_i\,r_l}\\
&+\sum_{i\in\Asing}\sum_{s\in\Asing} q_s\sum_{n=2}^{\infty}\sum_{\uomega' \in \Bscr_n(s, i)}p(\uomega')\log\norm{A^n(\uomega')\, r_s} \\
&-\sum_{l\in\Ainv}\sum_{s\in \Asing}q_s \sum_{\uomega\in\Bscr_1(s, l)} p(\uomega)\log\norm{A^1(\uomega)\,r_s} \\
\\
&= \sum_{l\in\Ascr}\sum_{s\in\Asing} q_s \, p_{l s}\, \log\norm{A_l\,r_s}\\
&+\sum_{l\in\Asing}\sum_{s\in\Asing} q_s\sum_{n=2}^{\infty}\sum_{\uomega \in \Bscr_n(s, l)}p(\uomega)\log\norm{A^n(\uomega)\, r_s} \\
&-\sum_{l\in\Ainv}\sum_{s\in \Asing}q_s \, p_{l s} \log\norm{A_l \,r_s} \\
\\
&= \sum_{l\in\Asing}\sum_{s\in\Asing} q_s \, p_{l s}\, \log\norm{A_l\,r_s}\\
&+\sum_{l\in\Asing}\sum_{s\in\Asing} q_s\sum_{n=2}^{\infty}\sum_{\uomega \in \Bscr_n(s, l)}p(\uomega)\log\norm{A^n(\uomega)\, r_s} \\
& = \sum_{l\in\Asing}\sum_{s\in\Asing} q_s\sum_{n=1}^{\infty}\sum_{\uomega \in \Bscr_n(s, l)}p(\uomega)\log\norm{A^n(\uomega)\, r_s} \, .
\end{align*} 
The first line turned into the fourth after re-denoting the index $i$ by $l$ and the index $l$ by $s$; the final equality follows since $(s, l)$ is the only word $\uom\in\Bscr_1 (s, l)$ and in this case $p(\uom)=p_{l s}$ and $A^1 (\uom)=A_l$.
The expression in the last line is exactly the formula obtained in Lemma~\ref{propL1} for $L_1 (\uA)$ so the proof of Furstenberg's formula is complete.
\end{proof}

\begin{remark}
We note that the classical Furstenberg's formula (i.e.~\cite[Theorem 8.5]{Fur63}) for random cocycles in $\GL_d (\R)$, or other more recent versions thereof, are obviously not applicable to this singular setting. Moreover, the probabilistic approach used by Furstenberg and Kifer to establish such results (see e.g.~\cite[Theorem 1.4]{FK83}) is not immediately applicable either, since the observable $\Psi$ is not continuous, not even bounded on $\Ascr \times \Proj$. That is why we had to employ an ad-hoc argument which uses the explicit formula of the stationary measure. 
\end{remark}

%\begin{remark}\label{stationary measure Bernoulli} The Bernoulli case can be treated similarly, but in a much more straightforward way; moreover, all relevant quantities have much simpler expressions. Let us summarize the main definitions and results. Let $(\uA, p)$ be a Bernoulli random cocycle of rank one.
%
%The Markov operator in this setting is $\Qop \colon L^\infty(\Pp^1) \to L^\infty(\Pp^1)$,
%$$\Qop \varphi (\hat v) := \sum_{i\in\Ascr} \varphi (\hat A_i \hat v) \, p_i .$$
%
%Given $n\ge 0$ and $s \in \Asing$, let $\Bscr_{n} (s)$ denote the set of $(n+1)$-tuples  $\uom=(\omega_0, \om_1, \ldots, \omega_{n})$ such that $\omega_0=s$ and 
%$\omega_i\in \Ainv$ for all $i=1, \ldots, n$.
%For such a word we write, as before, 
%$A^{n}(\uom):=A_{\omega_{n}}\, \ldots\, A_{\omega_2}\, A_{\omega_1}$  (with the convention that $A^0 (\uom)$ is the identity matrix) and denote the quantity
% $p (\uom):=p_{\omega_0} \, p_{\om_1} \cdots \, p_{\omega_{n}}$. 
%  
%With these notations we have the following explicit formula for the unique $\Qop$-stationary measure
%$\eta\in\Prob (\Pp^1)$:
%$$
%\eta =  \sum_{s \in \Asing} \sum_{n=0}^\infty
%\sum_{\uom\in\Bscr_n(s)}  p(\omega)\delta_{\hat A^n(\omega) \, \hat r_s} \, .
%$$
%
%We write $\Qop = \Qinv + \Qsing$, with $\Qinv \varphi (\hat v) := \sum_{i\in\Ainv} \varphi (\hat A_i \hat v) \, p_i$ and 
%$\Qsing \varphi (\hat v) := \sum_{i\in\Asing} \varphi (\hat r_i) \, p_i$. Note that $\Qsing$ is a projection to a constant function. This then easily implies by induction that for all $n\in\N$,
%\begin{equation}\label{Qop Iterates}
%\Qop^n = \Qinv^n + \Qsing\circ \Big(\sum_{i=0}^{n-1} \Qinv^i\Big)  \, .
%\end{equation}
%In particular, $\Qop^n - \Qinv^n$ takes any observable $\varphi$ to a constant function, which then implies the uniform ergodicity of the Markov operator, namely the fact that
%$$  \norm{  \Qop^n\varphi - \int\varphi\, d\eta }_\infty \leq C\, e^{-a\,n}\,\norm{\varphi}_\infty $$
%for all $n\in\N$ and  
%$\varphi\in L^\infty(\Pp^1)$.
%
%Finally, defining the observable $\psi \colon \Pp^1 \to [- \infty, \infty)$,
%$$\psi (\hat v) := \sum_{i\in\Ascr} p_i \, \log \frac{\norm{A_i v}}{\norm{v}} \, ,$$
%the Lyapunov exponent of the random cocycle $\uA$ is given by
%$$L_1 (\uA) = \int \psi (\hat v)  \, d \eta (\hat v) \, ,$$
%that is, a Furstenberg-type formula holds.
%\end{remark}
%


==> statistical-properties.tex <==

 Given the alphabet $\Ascr = \{1, \ldots, k\}$ and a partition $\Ascr = \Asing \sqcup \Ainv$ into two nonempty sets, consider the space $\cocycles$ of all $k$-tuples $\uA = (A_1, \ldots, A_k) \in \Mat_2^+ (\R)^k$ such that $\rank A_i = 1$ if $i \in \Asing$, $\det A_j > 0$ if $j\in\Ainv$ and $\hat r_i \neq \hat k_i$ for all $i\in\Asing$. Recall that we identify such a $k$-tuple $\uA$ with the locally constant map $A \colon X \to \Mat_2^+ (\R)$, $A (\om) = A_{\om_0}$, where $\om = \{\om_n\}_{n\in \Z} \in X = \Ascr^\Z$. 
 
 %there are no null words, that is,  $A_{i_1} \cdots A_{i_l} \neq 0$ for all $l\in \N$ and $i_1, \ldots, i_l \in \Ascr$.


Given a probability vector $p = (p_1, \ldots, p_k)$ with $p_i > 0$ for all $i$, the   $k$-tuple $\uA = (A_1, \ldots, A_k)$ determines the random linear cocycle 
$F \colon X \times \R^2 \to X \times \R^2$, $F (\om, v) = (\sigma \om, A (\om) v) = (\sigma \om, A_{\om_0} \, v)$
where $X$ is endowed with the product probability $\mu = p^\Z$.
As before, we also identify the cocycle $F$ with the tuple $\uA = (A_1, \ldots, A_k)$.

The Markov operator in this setting is $\Qop \colon L^\infty(\Pp^1) \to L^\infty(\Pp^1)$,
$$\Qop \varphi (\hat v) := \sum_{i\in\Ascr} \varphi (\hat A_i \hat v) \, p_i .$$

Given $n\ge 0$ and $s \in \Asing$, let $\Bscr_{n} (s)$ denote the set of $(n+1)$-tuples  $(s \uom)$ where $\uom=(\om_1, \ldots, \omega_{n}) \in \Ainv^n$.  
For such a word we write, as before, 
$A^{n}(s \uom):=A_{\omega_{n}}\, \ldots\, A_{\omega_2}\, A_{\omega_1}$  (with the convention that $A^0 (s \uom)$ is the identity matrix) and denote the quantity
 $p (\uom):= p_{\om_1} \cdots \, p_{\omega_{n}}$ 
 
 Let $q:= \sum_{i\in\Asing} p_i < 1$ and note that
\begin{align}\label{inca o suma}
\sum_{s \in \Asing} p_s \sum_{n=0}^\infty
	\sum_{\uomega \in \Ainv^n}  p(\uomega) = \sum_{s \in \Asing} p_s \sum_{n=0}^\infty (1-q)^n = q \, \frac 1 q = 1 .
\end{align}
  
With these notations we have the following explicit formula for the unique $\Qop$-stationary measure
$\eta\in\Prob (\Pp^1)$ (its derivation is quite straightforward compared to the Markov case, so we omit it):
$$
\eta =  \sum_{s \in \Asing} \sum_{n=0}^\infty
\sum_{\uom\in\Bscr_n(s)}  p(\uomega)\delta_{\hat A^n(s \uomega) \, \hat r_s} \, .
$$

We write $\Qop = \Qinv + \Qsing$, with $\Qinv \varphi (\hat v) := \sum_{i\in\Ainv} \varphi (\hat A_i \hat v) \, p_i$ and 
$\Qsing \varphi (\hat v) := \sum_{i\in\Asing} \varphi (\hat r_i) \, p_i$. Note that $\Qsing$ is a projection to a constant function. This then easily implies by induction that for all $n\in\N$,
\begin{equation}\label{Qop Iterates}
\Qop^n = \Qinv^n + \Qsing\circ \Big(\sum_{i=0}^{n-1} \Qinv^i\Big)  \, .
\end{equation}
In particular, $\Qop^n - \Qinv^n$ takes any observable $\varphi$ to a constant function, which then implies the uniform ergodicity of the Markov operator, namely the fact that
\begin{equation}\label{eq1001}
  \norm{  \Qop^n\varphi - \int\varphi\, d\eta }_\infty \leq C\, e^{-a\,n}\,\norm{\varphi}_\infty 
 \end{equation} 
for all $n\in\N$ and  
$\varphi\in L^\infty(\Pp^1)$.

Finally, defining the observable $\psi \colon \Pp^1 \to [- \infty, \infty)$,
$$\psi (\hat v) := \sum_{i\in\Ascr} p_i \, \log \frac{\norm{A_i v}}{\norm{v}} \, ,$$
the Lyapunov exponent of the random cocycle $\uA$ is given by
\begin{equation}\label{F formula 10}
L_1 (\uA) = \int \psi (\hat v)  \, d \eta (\hat v) \, ,
\end{equation}
that is, a Furstenberg-type formula holds.

The goal of this section is to establish a large deviations type (LDT) estimate and a central limit theorem (CLT) for Lebesgue almost every  cocycle $\uA \in \cocycles$. This will be obtained as a consequence of a stronger result essentially saying that if $t\mapsto\uA_t$ is a one-parameter family of such cocycles satisfying a positive winding condition, then an LDT estimate and a CLT hold for Lebesgue almost every parameter $t$. By general results, see Cai, Duarte, Klein~\cite{CDK-paper3}, such limit laws hold as soon as an associated stochastic dynamical system / Markov operator satisfies an appropriate mixing condition. We will use a parameter elimination argument to show that for Lebesgue a.e. parameter $t$, the Markov operator corresponding to $\uA_t$ satisfies the desired mixing condition. 

For simplicity of exposition, all statements in this section will be proven in the Bernoulli setting, but it will be clear that the arguments easily extend to the mixing Markov shift setting. 



In order to apply the general results in~\cite{CDK-paper3} we need to associate to a given cocycle $\uA\in\cocycles$ a Markov operator on a slightly larger space, namely
$\bar{\Qop} \colon L^\infty(\Ascr \times \Pp^1) \to L^\infty(\Ascr \times \Pp^1)$ defined by
$$\bar{\Qop}\varphi(j,\hat{v}) = \sum_{i=1}^{k}p_i \varphi(i,\hat{A}_j \hat v) \, .$$

Consider the projection $\pi \colon L^\infty(\Ascr \times \Pp^1) \to L^\infty(\Ascr)$ given by 
$$
\pi \varphi (\hat{v}) = \sum_{i=1}^{k}p_i  \varphi(i,\hat{v}) = \int_\Ascr \varphi (i, \hat v) \, d p (i) \, .
$$

Then the Markov operators $\bar \Qop$ and  $\Qop$ are related as follows.






\begin{lemma}\label{Diagrama}
The following diagram is commutative:
\[ \begin{tikzcd}
L^\infty(\Ascr \times \Pp^1) \arrow{r}{\bar{\Qop}} \arrow[swap]{d}{\pi} & L^\infty(\Ascr \times \Pp^1) \arrow{d}{\pi} \\%
L^\infty( \Pp^1) \arrow{r}{\Qop} & L^\infty(\Pp^1)
\end{tikzcd}
\]
That is, $\pi \circ \bar{\Qop}=\Qop \circ \pi$ and inductively, $\pi \circ \bar{\Qop}^n=\Qop^n \circ \pi$ for all $n\in\N$.
\end{lemma}

\begin{proof}
Let $\varphi \in L^\infty(\Ascr \times \Pp^1)$. Then,

$$\pi \circ \bar{Q} (\varphi) (\hat v) = \sum_{j=1}^k p_j \bar{Q} \varphi (j, \hat v) 
= \sum_{j=1}^k \sum_{i=1}^k p_j \, p_i \, \varphi (i, \hat A_j \hat v) ,$$
while
$$Q \circ \pi  (\varphi) (\hat v) = \sum_{j=1}^k p_j \pi \varphi (\hat A_j, \hat v) 
= \sum_{j=1}^k \sum_{i=1}^k p_j \, p_i \, \varphi (i, \hat A_j \hat v) $$
which establishes the claim.
\end{proof}

\begin{corollary}\label{cor strong mixing}
The measure $p \times \eta$ is $\bar{\Qop}$-stationary and $\bar{Q}$ is strongly mixing. More precisely, there exist constants $c$ and $C$ such that
$$
\norm{\bar{Q}^n \varphi - \int \varphi \; d\mu d\eta}_\infty \leq C e^{-cn}\norm{\varphi}_\infty \quad \quad \forall \; n \in \N, \; \forall \; \varphi \in L^\infty(\Ascr \times \Pp^1) .
$$
\end{corollary}

\begin{proof} For any observable $\varphi \in L^\infty(\Ascr \times \Pp^1)$ we have
 \begin{align*}
 \iint \bar \Qop \varphi (i, \hat v) d p(i) d \eta (\hat v) &= \int \pi (\bar \Qop \varphi) (\hat v) d \eta (\hat v) 
 = \int \Qop (\pi \varphi) (\hat v) d \eta (\hat v) \\
 &= \int \pi \varphi (\hat v) d \eta (\hat v) = 
 \iint \varphi (i, \hat v) d p (i) d \eta (\hat v) ,
 \end{align*}
 which shows that $p \times \eta$ is $\bar{\Qop}$-stationary. 
Moreover,
\begin{align*}
\bar{\Qop}^{n+1} \varphi (j,\hat{v}) &= \bar{\Qop} \bar{\Qop}^n \varphi (j,\hat{v}) = \sum_{i=1}^k p_i \bar{\Qop}^n \varphi (i,\hat{A}_j \hat{v}) \\
&= \pi (\bar{\Qop}^n \varphi)  (\hat{A}_j \hat{v}) = \Qop^n(\pi \varphi)(\hat{A}_j \hat{v}).
\end{align*}

Since by~\eqref{eq1001} the operator $\Qop$ is strongly mixing, the last term converges uniformly and exponentially fast to $\int \pi \varphi \; d\eta = \iint \varphi \; d p d\eta$, thus showing the strong mixing of $\bar \Qop$.
\end{proof}


Let $\Lambda \subset \R$ be a compact interval (normalized to have length $1$)  and let $A\colon \Lambda \to \cocycles$ be a smooth map. We think of this map as a one-parameter family of random cocycles so we use the subscript notation $t \mapsto A_t$. For its components we write $A_t (i)$ instead of $(A_t)_i$, while the fiber iterates are denoted by
$$A_t^n (\om) = A_t (\om_{n}) \cdots A_t (\om_1) \, .$$

For every parameter $t\in\Lambda$, denote by $\Qop_t$ and $\bar \Qop_t$ the Markov operators corresponding to the cocycle $A_t$ (defined as above). Moreover, let $\eta_t \in \Prob (\Pp^1)$ be the unique $\Qop_t$-stationary measure. All the results proven above for a given cocycle $A\in\cocycles$, namely the explicit formula of the stationary measure, Furstenberg's formula and the strong mixing of the Markov operator, apply to $A_t$ for all $t\in\Lambda$; since the probability vector $p = (p_1, \ldots, p_k)$ and the singular/invertible symbols do not change, all the mixing parameters are uniform in $t$. Finally, recall that the stationary measure is given by:
$$
\eta_t =  \sum_{s \in \Asing} p_s \, \sum_{n=0}^\infty
\sum_{\uom \in \Ainv^n}  p(\uomega) \delta_{\hat A_t^n(s\uomega) \, \hat r_s} \, .
$$   

\subsection{Assumptions}\label{assumptions} We assume that the family of cocycles $\Lambda \ni t \mapsto A_t$ is positively winding (see Definition~\ref{def pos winding}) and that its singular components are constant. More precisely, we impose the following conditions on the smooth map  $t \mapsto A_t$:
\begin{enumerate}
\item[(A1)] For all $i\in \Asing$, $A_t (i) \equiv A_i$.

\item[(A2)] There is $c_0 > 0$ such that for all $t \in \Lambda$, $j \in \Ainv$ and $\hat v \in \Pp^1$ we have
$$\frac{A_t (j)\, v \wedge \frac{d}{d t} \, A_t (j) v }{\norm{A_t (j) \, v}^2}   \ge c_0 \, .$$
\end{enumerate}

\begin{remark}By~\cite[Proposition 3.1]{BCDFK}, the quantity in item (A2) above, which we refer to as the rotation speed of the map $t\mapsto A_t$, can be characterized by
$$\frac{d}{d t} \, \hat A_t (j) \hat v = \frac{d}{d t} \, \frac{A_t (j) v}{\norm{A_t (j) v}} = \frac{A_t (j)\, v \wedge \frac{d}{d t} \, A_t (j) v }{\norm{A_t (j) \, v}^2} \, .$$
\end{remark} 

\begin{remark}
A more general version of the winding condition requires that the inequality  in assumption (A2) above holds for some iterate $\uA_t^{n_0}$ of the cocycle.  For simplicity we assume that $n_0=1$.

Moreover, if the assumption (A2) holds, then there exists $c_1 > 0$ that only depends on the map $A$, such that $\forall n \in \N$, $\forall \om \in \Ainv^n$, $\forall \hat{v} \in \Pp^1$, we have
\begin{equation} \label{Winding for An}
\frac{d}{dt} \frac{A_t^n(\om)v}{\norm{A_t^n(\om)v}} \geq c_1.
\end{equation}

In other words, if  $A_t$ is a family of positively winding cocycles, then so is $A_t^n$ for every $n \in \N$, with rotation speed uniformly (in $n$) bounded from below. For a proof of this statement see~\cite[Section 3.1]{BCDFK}, specifically 
Propositions 3.3 and 3.4.
\end{remark} 

\begin{example}
Given any tuple $\underline{A} = (A_1, \ldots, A_k) \in \cocycles$, the one-parameter family $\left[ - \frac{1}{2}, \frac{1}{2} \right] \mapsto A_t \in \Matdm^k$,
$A_t (i) = A_i$ if $i \in \Asing$ and 
$$A_t (j) = A_j \, R_{2 \pi t} = \begin{bmatrix} \cos 2 \pi t & - \sin 2 \pi t \\ \sin 2 \pi t & \cos 2 \pi t \end{bmatrix} \quad \text{if } \, j \in \Ainv $$
satisfies the assumptions (A1) and (A2) above and passes through $\underline{A}$.
\end{example}

%\begin{example}
%Schrodinger example
%\end{example}

\subsection{Some technical estimates}

In order to simplify the exposition in the estimates to follow, we will write $a \less b$ if there is some absolute or at least context universal constant $C < \infty$ such that $a \le C \, b$. Moreover, for an arc $\hat I \subset \Pp^1$, $m (\hat I)$ denotes its length, while $\Leb (E)$ stands for the Lebesgue measure of a subset $E$ of the real line. 





\begin{lemma} \label{lemma finite arcs}
Given any $\varepsilon >0$, the set 
$$
\hat{I}_\varepsilon \colon = \left \{ \hat{v} \in \Pp^1 \colon \norm{A_i \frac{v}{\norm{v}}} < \varepsilon \text{ for some } i \in \Asing \right \}
$$
is a finite union of arcs with  $m(\hat{I}_\varepsilon) \less \varepsilon$.
\end{lemma}

\begin{proof}
Let $i \in \Asing$ and consider the normalized directions $r_i$ and $k_i$ of the range and kernel of $A_i$, respectively, such that  $\norm{k_i} = \norm{r_i}=1$. Given any vector $v \in \R^2$, we can write $v = \alpha_1 r_i + \alpha_2k_i$.

Hence, 
$$
\norm{A_i \frac{v}{\norm{v}}} = \frac{| \alpha_1 |}{\norm{v}}.
$$
Therefore, $\norm{A_i \frac{v}{\norm{v}}} < \varepsilon$ in a small interval around each kernel $k_i$. Moreover $\hat{I}_\varepsilon$ is a finite union of arcs of length approximately $2\varepsilon$ each. Hence $m(\hat{I}_\varepsilon) \lesssim \varepsilon$.
\end{proof}


\begin{lemma} \label{lemma Leb measure of t in I}
Given any arc $\hat I \subset \Pp^1$,  $n\in\N$, $\om \in \Ainv^n$ and $\hat v \in \Pp^1$ we have
$$
\Leb \left\{ t \in \Lambda \colon \hat{A}^n_t(\om) \hat{v} \in \hat{I} \right\} \le  \frac{m(\hat{I})}{c_1} .
$$
\end{lemma}

\begin{proof} Since the projective line $\Pp^1$ is one dimensional, we may regard the map $\Lambda \ni t \mapsto  \hat{A}^n_t(\om) \hat{v}$ as a real valued map, whose derivative (because of the winding condition) is bounded from below by $c_1$. The result then follows using basic calculus (the mean value theorem).
\end{proof}


Consider the maps $\varphi_t \colon \Ascr \times \Pp^1 \to [-\infty, \infty)$ and $\psi_t \colon \Pp^1 \to[-\infty, \infty)$ given by
$$
\varphi_t(i,\hat{v}) := \log \norm{A_t(i) \frac{v}{\norm{v}}} \, \text{ and } \, \psi_t(\hat{v})= \sum_{i \in \Ascr} p_i\varphi_t(i,\hat{v}) = \int_\Ascr \varphi_t (i, \hat v) d p(i) .
$$

Let $c=c(A)$ be a constant that satisfies

\begin{enumerate}
\item[(i)] $e^{-c } \le \norm{A_t(j)} \leq e^c \quad \forall t \in \Lambda \text{ and } \forall j \in \Ainv$.
\item[(ii)] $\norm{A_i} \leq e^c \quad \forall i \in \Asing$. 
\item[(iii)] $\norm{A_ir_l} \geq e^{-c} \quad \forall i,l \in \Asing $.
\end{enumerate}

Such a constant exists by the compactness of $\Lambda$ and the fact that there are no null words. It follows that for all $j \in \Ainv$  and  $\hat{v} \in \Pp^1$ we have $\abs{  \varphi_t(j,\hat{v}) } \le c$. Moreover, the upper bound $\varphi_t(j,\hat{v}) \le c$  holds for every $j \in \Ascr$ and  $\hat{v} \in \Pp^1$.


%$$
%|\varphi_t(j,\hat{v})| \leq c \quad \text{and} \quad |\psi_t(\hat{v})| \leq c .
%$$
%Moreover, the upper bounds $\varphi_t(j,\hat{v}) \leq c$ and  $\psi_t(\hat{v}) \leq c$ hold for every $j \in \Ascr$ and  $\hat{v} \in \Pp^1$.

%Consider the set 
%\begin{align*}
%Z &= \left \{ \hat{v} \in \Pp^1 \colon \hat{A}^n (\om)\hat{v} =k_i  \, \text{ for some }  n \ge 1 \; \om \in \Ainv^n \; i \in \Asing   \right \} \\
%&= \left \{  \hat{A}^n(\om)^{-1}k_i \colon \om \in \Ainv^n , \; n >0, \; i \in \Asing \right\}
%\end{align*}
%
%Then, by the definition of $\eta$, we conclude that $\eta(Z)=0$. 

\begin{lemma} \label{lem exp small measure}
There is  $C < \infty$ which depends on the constants $c, c_1$, so only on $A$ such that the following hold. \begin{enumerate}
\item[(i)] For all $n\in\N$, $\om \in \Ainv^n$,  $i \in \Asing$, $\hat v \in \Pp^1$ and $N\ge 0$ we have
$$
\Leb \{ t \in \Lambda \colon \varphi_t(i, \hat{A}^n_t(\om)\hat{v}) < - N \} \le C \, e^{-N} \, .
$$
Moreover, 
$$
\int_{\Lambda} \varphi_t^2(i,\hat{A}^n_t(\om)\hat{v}) \; dt \le C .
$$

\item[(ii)] For all  $n\in\N$,  $\om \in \Ascr^n$, $i, s \in \Asing$  and $N\ge 0$ we have
$$
\Leb \{ t \in \Lambda \colon \varphi_t (i,\hat{A}^n_t(\om)\hat{r}_s) < - N \} \le C \, e^{-N} \, .
$$
Moreover, 
$$
\int_{\Lambda} \varphi_t^2(i,\hat{A}_t^n(\om)\hat{r}_s) \; dt \le C .
$$

\item[(iii)] Furthermore, for all $i\in\Ascr$, $\om \in X$ and $n\in\N$,
$$\int_\Lambda \int_{\Pp^1} \varphi_t^2 (i, \hat A_t^n (\om) \hat v) \, d \eta_t (\hat v) \, d t \le C .$$

In particular,
$$\int_\Lambda \int_{\Pp(\R^2)} \psi_t^2 (\hat A_t^n (\om) \hat v) \, d \eta_t (\hat v) \, d t \le C .$$

%\item[(ii)]For any $\om \in \Ascr^n$ and $v \notin Z$ ,
%$$
%\Leb \{ t \in \Lambda \colon \varphi_t (i,\hat{A}^n_t(\om)\hat{v}) <-x \} <ne^{-x}.
%$$
%
%Moreover, 
%$$
%\int_{\Lambda} \varphi_t^2(i,\hat{A}_t^n(\om)\hat{v}) \; dt \lesssim n+c^2.
%$$
%\item[(iii)] For any $\om \in \Ascr^n$ and $s \in \Asing Z$,
%$$
%\int_{\Lambda} \psi_t^2(\hat{A}^n_t(\om)\hat{r}_s) \; dt \lesssim n+c^2.
%$$

%\item[(iii)] For any $\om \in \Ascr^n$ and $v \notin Z$,
%$$
%\Leb \{ t \in \Lambda \colon \psi_t (\hat{A}^n_t(\om)\hat{v}) <-x \} <ne^{-x}.
%$$
%Moreover,
%$$
%\int_{\Lambda} \psi_t^2(\hat{A}^n_t(\om)\hat{v}) \; dt \lesssim n+c^2.
%$$
\end{enumerate} 
\end{lemma}

\begin{proof}
(i) If $i\in\Asing$ then $\varphi_t (i, \hat w) < - N$ holds if and only if $\norm{A_i  \frac{w}{\norm{w}}} < e^{- N}$. By Lemma~\ref{lemma finite arcs} the set of such points $\hat w$ is a finite union of arcs with total measure of order $\varepsilon := e^{-N}$, and by Lemma~\ref{lemma Leb measure of t in I} the measure of the set of parameters $t$ for which $\hat{A}^n_t(\om)\hat{v}$ belongs to these arcs is $\less \varepsilon$. This proves the first statement in item (i).  

For the second statement, note that
\begin{align*}
&\int_{\Lambda} \varphi_t^2(i,\hat{A}^n_t(\om)\hat{v}) \; dt = \int_0^\infty \Leb \{ t \in \Lambda \colon \varphi_t^2 (i, \hat{A}^n_t(\om)\hat{v}) \geq x \} \; dx\\
&= \int_0^{2 c^2} \Leb \{ t \in \Lambda \colon \varphi_t^2 (i, \hat{A}^n_t(\om)\hat{v}) \geq x \} \; dx \\
&+ \int_{2 c^2}^{\infty} \Leb \{ t \in \Lambda \colon \varphi_t^2 (i, \hat{A}^n_t(\om)\hat{v}) \geq x \} \; dx \\
&\leq 2 c^2 + \int_{2 c^2}^{\infty} \Leb \{ t \in \Lambda \colon  \varphi_t (i, \hat{A}^n_t(\om)\hat{v})  \le - \sqrt{x}  \} \; dx \\
&\less c^2 + \int_{2 c^2}^{\infty} e^{-\sqrt{x}} \; dx \less 1 .
\end{align*}

The bound in the penultimate line above holds because $\Lambda$ has length one and, moreover,  the upper bound $ \varphi_t(i,\hat{w}) \leq c$ is valid for all $\hat w \in \Pp^1$, so that  $\varphi_t (i,\hat{A}^n_t(\om)\hat{v}) \le c < \sqrt{x}$ when $x\ge2c^2$. 

\smallskip

 (ii) Note that if $\om \in \Ainv^n$, then the statement follows from item (i). The difference here is that we consider any word $\om$, invertible or not, but begin with a singular vector, namely $r_s$. 
 
Let $\om = (\om_{0}, \ldots, \om_{n-1})  \notin \Ainv^n$. We split the argument into two cases: either $\om_{n-1} \in \Asing$ or else $\om_{n-1} \in \Ainv$ but there is $0 \leq j \leq n-2$ such that $\om_j \in \Asing$.

%If $\om_{n-1} \in \Asing$, then 
%$$
%\hat{A}_t^n(\om)r_s = \hat{A}_t(\om_{n-1})\hat{A}_t^{n-1}(\om)\hat{r}_s = \hat{r}_{\om_{n-1}}.
%$$
%
%Thus, we conclude that 
%$$
%\varphi_t(i,\hat{A}^n_t(\om)\hat{r}_s) = \log \frac{\norm{ \hat{A}_i \hat{r}_{\om_{n-1}} }   }{\hat{r}_{\om_{n-1}}} \geq -c > -x.
%$$ 
%
%Hence $| \varphi_t(i,\hat{A}^n_t(\om)\hat{r}_s) | \leq c$ for every $t \in \Lambda$ and
%$$
%\int_{c^2}^\infty \Leb \{ t \in \Lambda \colon |\varphi_t(i,\hat{A}^n_t(\om)\hat{r}_s)| > \sqrt{x}  \} \; dx =0.
%$$
%
%This concludes the first case. Now assume that $\om_{n-1} \in \Ainv$ and there is $0 \leq j \leq n-2$ such that $\om_j \in \Asing$. Let $n'$ be the largest index that belongs to $\Asing$ and let $\om' = \{ \om_{n'+1}, \dots , \om_{n-1} \} \in \Ainv^{n-n'-1}$.
%
%Then 
%$$
%\hat{A}^n_t(\om)\hat{r}_s = \hat{A}_t^{n-n'-1}(\om')\hat{A}_{\om_{n'}}\hat{A}^{n'}_t(\om)\hat{r}_s = \hat{A}^{n-n'-1}_t \hat{r}_{\om_{n'} }.
%$$
%
%Thus, $\varphi_t(i, \hat{A}_t(\om)\hat{r}_s ) = \varphi_t(i, \hat{A}_t^{n-n'-1}(\om')\hat{r}_{\om_{n'}})$, with $\om' \in \Ainv$, hence (i) is applicable and the conclusion follows.

If $\om_{n-1} \in \Asing$, then 
$$
\hat{A}_t^n(\om)\hat{r_s} = \hat{A}_t(\om_{n-1})\hat{A}_t^{n-1}(\om)\hat{r_s} = \hat A_{\om_{n-1}} \, \hat{A}_t^{n-1}(\om)\hat{r_s} = \hat{r}_{\om_{n-1}}.
$$

Then by the choice of the constant $c$, for all parameters $t \in \Lambda$,
$$
\varphi_t (i, \hat{A}^n_t(\om)\hat{r_s}) = \log \norm{ \hat{A}_i \hat{r}_{\om_{n-1}} }  \geq -c ,
$$ 
so the set $\{ t \in \Lambda \colon \varphi_t (i,\hat{A}^n_t(\om)\hat{r}_s) < - N \}$ becomes empty for $N \ge c$ and the statement follows trivially.



If  $\om_{n-1} \in \Ainv$ and $\om_j \in \Asing$ for some index $0 \leq j \leq n-2$, let $n'$ be the largest such index and let $\om' :=  (\om_{n'+1}, \dots , \om_{n-1})\in \Ainv^{n-n'-1}$.
Then 
$$
\hat{A}^n_t(\om)\hat{r}_s = \hat{A}_t^{n-n'-1}(\om')\hat{A}_{\om_{n'}}\hat{A}^{n'}_t(\om)\hat{r}_s = \hat{A}^{n-n'-1}_t (\om') \hat{r}_{\om_{n'} }.
$$
Thus $\varphi_t(i, \hat{A}_t^n (\om)\hat{r}_s ) = \varphi_t(i, \hat{A}_t^{n-n'-1}(\om')\hat{r}_{\om_{n'}})$, with $\om' \in \Ainv^{n-n'-1}$, hence item (i) is applicable and the conclusion follows.

(iii) If $i \in \Ainv$ the statement is obvious since $\varphi_t^2 (i, \hat w) \le c^2$ for all $(t, \hat w) \in \Lambda \times \Pp^1$. Let us then fix $i\in\Asing$. Using the explicit formula of $\eta_t$ we have
\begin{align*}
&\int_\Lambda \int_{\Pp^1} \varphi_t^2 (i, \hat A_t^n (\om) \hat v) \, d \eta_t (\hat v) \, d t  \\
& =  \sum_{s \in \Asing}p_s \sum_{j=0}^\infty \sum_{\uom \in \Ainv^j} p(\uom) \int_{\Lambda} \varphi_t^2  (i, \hat A_t^n (\om) \, \hat{A}_t^j (s\uom)   \hat{r}_s) \, dt\\
& =  \sum_{s \in \Asing}p_s \sum_{j=0}^\infty \sum_{\uom \in \Ainv^j} p(\uom) \int_{\Lambda} \varphi_t^2 (i,\hat{A}^{n+j}_t(s\uom \om)\hat{r}_s ) \, dt\\
& \le \sum_{s \in \Asing}p_s \sum_{j=0}^\infty \sum_{\uom \in \Ainv^n} p(\uom) \, C = C,
\end{align*}
where the inequality in the last line follows from item (ii) above and the last equality comes from~\eqref{inca o suma}.
\end{proof}



%Now we proceed to prove (iii).  The first statement follows from (ii), since
%for every $i \in \Asing$ it holds
%$$
%\Leb \{ t \in \Lambda \colon \varphi_t (i,\hat{A}^n_t(\om)\hat{v}) <-x \} <ne^{-x}.
%$$ 
%
%For the second, note that
%$$
%\psi_t^2(\hat{v}) = \left( \sum_{i \in \Ascr} p_i \varphi_t(i,\hat{v}) \right)^2 \leq \sum_{i \in \Ascr} p_i \varphi_t^2(i,\hat{v}).
%$$ 
%Therefore, (iii) follows from the previous items, since
%$$
%\int_{\Lambda} \psi_t^2 (\hat{A}_t^n(\om) \hat{v}) \; dt \leq \sum_{i \in \Ascr} p_i \int_{\Lambda} \varphi_t^2(i,\hat{A}^n_t(\om)\hat{v}) \; dt \lesssim n+c^2.
%$$
%\end{proof}

Let $\tilde \eta \in \Prob (\Lambda \times \Pp^1)$ be the probability measure whose disintegration relative to the Lebesgue measure on $\Lambda$ is $\{\eta_t\}$, that is, the measure characterized by
$$\int \phi (t, \hat v) \, d \tilde\eta (t, \hat v) = \int_\Lambda \int_{\Pp^1}  \phi (t, \hat v) \, d \eta_t (\hat v) \, d t \quad \forall \phi \in L^\infty (\Lambda \times \Pp^1) \, .$$



\begin{lemma}\label{lema 10}
Given $i \in \Ascr$, $n\in \N$, $N > c$ and $\om \in X$, let  
\begin{align*}
P_{i, n, N}(\om) : = \left\{  (t, \hat{v}) \colon \varphi_t(i, \hat{A}^n_t(\om)\hat{v}) < -N  \right\} .
\end{align*}

Then $\tilde{\eta} (P_{i, n, N}(\om)) \le C   e^{-N}$.
\end{lemma}

\begin{proof} 
If $i\in\Ainv$ then $\varphi_t(i, \hat w) \ge - c > - N$ for all $\hat w \in \Pp^1$, so $P_{i, n, N}(\om)$ is empty. We then fix $i \in\Asing$ and note that 
\begin{align*}
 \tilde{\eta}(P_{i, n, N}(\om)) &= \int_{\Lambda} \int_{\Pp^1} \ind_{P_{i, n, N}(\om)} (t,\hat{v}) \; d\eta_t(\hat{v}) dt \\
 &= \sum_{s \in \Asing}p_s \sum_{j=0}^\infty \sum_{\uom \in \Ainv^j} p(\uom) \int_{\Lambda} \ind_{P_{i, n, N}(\om)} (t, \hat{A}_t^j (s\uom) \hat{r}_s) \; dt.
\end{align*}

Moreover,
\begin{align*}
(t, \hat{A}_t^j (s\uom) \hat{r}_s) \in P_{i, n, N}(\om) &\Longleftrightarrow \varphi_t(i, \hat{A}^n_t(\om)\hat{A}^j_t(s\uom)\hat{r}_s) <-N  \\
&\Longleftrightarrow \varphi_t(i,\hat{A}^{n+j}_t(s\uom \om)\hat{r}_s ) < -N.
\end{align*} 

By Lemma~\ref{lem exp small measure} item (ii), for all $j \in \N$,
\begin{align*}
\int_{\Lambda} \ind_{P_{i, n, N}(\om)} (t, \hat{A}^j_t(s\uom)\hat{r}_s) \; dt = \Leb\{ t \colon \varphi_t(i, \hat{A}^{n+j}_t(s\uom \om)\hat{r}_s <-N \} \lesssim e^{-N}
\end{align*}
and the conclusion follows from~\eqref{inca o suma}.
\end{proof}

Given any $N>c$, consider the truncation
$$\varphi_{t, N} := \max \left\{ \varphi_t, - N \right\} \, .$$
Note that $\varphi_{t, N} \in L^\infty(\Ascr\times\Pp^1)$ (a property that does not hold for $\varphi_t$) and $\norm{\varphi_{t, N}}_\infty \le N$. Moreover, 
$\varphi_t (i, \hat v) = \varphi_{t, N} (i, \hat v)$ if and only if $i\in\Ainv$ or else $i\in\Asing$ and $\varphi_t (i, \hat v) < - N$.


\begin{lemma} \label{lemma Estimates phi and psi} 
For all $i\in\Ascr$, $n\in\N$, $N > c$ and $\om\in X$ we have
$$
\int_{\Lambda} \int_{\Pp^1} \abs{ \varphi_t (i, \hat A_t^n (\om) \hat v) -  \varphi_{t, N} (i, \hat A_t^n (\om) \hat v)} \, d\eta_t (\hat{v}) \, dt \less e^{-N/3} \, .
$$
\end{lemma}

\begin{proof} The statement is obvious when $i\in\Ainv$ since in this case $\varphi_t (i, \hat w) = \varphi_{t, N} (i, \hat w)$ for all $\hat w \in \Pp^1$.

We  fix $i\in\Asing$ and recall that $\varphi_t (i, \hat A_t^n (\om) \hat v) \neq \varphi_{t, N} (i, \hat A_t^n (\om) \hat v)$ if and only if $\varphi_t (i,  \hat A_t^n (\om) \hat v) < - N$, that is, if and only if  $(t, \hat v) \in P_{i, n, N} (\om) =: P_N$, which by Lemma~\ref{lema 10} is a set of $\tilde \eta$-measure $\less e^{- N}$. Then 
\begin{align*}
& \int_{\Lambda} \int_{\Pp^1} \abs{ \varphi_t (i,  \hat A_t^n (\om) \hat v) -  \varphi_{t, N} (i,  \hat A_t^n (\om) \hat v)} \, d\eta_t (\hat{v}) \, dt \\
& = \int_{\Lambda \times \Pp^1} \abs{ \varphi_t (i,  \hat A_t^n (\om) \hat v) -  \varphi_{t, N} (i,  \hat A_t^n (\om) \hat v)} \, \ind_{P_N} (t, \hat v) \,  d \tilde \eta (t, \hat v)\\
& \le \norm{g (t, \hat v)}_{L^2 (\tilde \eta)} \, \,  \tilde \eta (P_N)^{1/2}
\end{align*}
where $g (t, \hat v) :=  \varphi_t (i,  \hat A_t^n (\om) \hat v) -  \varphi_{t, N} (i,  \hat A_t^n (\om) \hat v)$ and we used Cauchy-Schwarz in the last inequality above. 

Moreover, by Lemma~\ref{lem exp small measure} item (iii),
$$\norm{g (t, \hat v)}_{L^2 (\tilde \eta)} \le \norm{\varphi_t (i,  \hat A_t^n (\om) \hat v)}_{L^2 (\tilde \eta)} + \norm{\varphi_{t, N} (i,  \hat A_t^n (\om) \hat v)}_{L^2 (\tilde \eta)} \le \sqrt{C} + N .$$

Thus
$$\int_{\Lambda} \int_{\Pp^1} \abs{ \varphi_t (i,  \hat A_t^n (\om) \hat v) -  \varphi_{t, N} (i,  \hat A_t^n (\om) \hat v)} d\eta_t (\hat{v}) dt \less ( \sqrt{C} + N)  e^{-N/2} \less e^{-N/3} $$
which completes the proof.
\end{proof}

%\begin{lemma} \label{lemma B_N}
%Let $n >0$ and $N >c$. 
%\begin{enumerate}
%\item[(i)] For all $\om \in \Ascr$, there is $B_{\varphi,n,N}(\om) \subset \Lambda \times \Pp^1$  with $\tilde{\eta}(B_{\varphi,n,N}) \lesssim n^2 e^{-N}$
%such that 
%$$
%\varphi_t(\om, \hat{A}^n_t(\om)\hat{v}) = \varphi_{t,N}(\om, \hat{A}^n_t(\om)\hat{v})
%$$
%for every $(t, \hat{v}) \notin B_{\varphi,n,N}(\om)$. \\
%In particular,
%$
%S_n\varphi_t(\om, \hat{v}) = S_n \varphi_{t,N}(\om, \hat{v})
%$
%for every $(t, \hat{v}) \notin B_{\varphi,n,N}(\om)$.
%\item[(ii)] For all $\om \in \Ascr$, there is $B_{\psi,n,N}(\om) \subset \Lambda \times \Pp^1$ with $\tilde{\eta}(B_{\psi,n,N}(\om)) \lesssim n^2 e^{-N}$ such that
%$$
%\psi_t(\hat{A}^n_t(\om)\hat{v}) = \psi_{t,N}( \hat{A}^n_t(\om)\hat{v})
%$$
%for every $(t, \hat{v}) \notin B_{\psi,n,N}(\om)$. \\
%In particular, $\Qop_t^n \psi_{t}(\hat{v}) = \Qop_t^n \psi_{t,N}(\hat{v})$ for every $(t, \hat{v}) \notin B_{\psi,n,N}(\om)$.
%\end{enumerate}
%
%\end{lemma}
%
%\begin{proof}
%We start with the proof of (i). By definition,
%\begin{align*}
%&S_n \varphi_t(\om, \hat{v}) = \sum_{m=0}^{n-1} \varphi_t(\om_m, \hat{A}^m_t(\om)\hat{v}) \quad \text{and} \\
%&S_n \varphi_{t,N}(\om, \hat{v})= \sum_{m=0}^{n-1}\varphi_{t,N} (\om_m, \hat{A}^m_t(\om)\hat{v}).
%\end{align*}
%
%If $\om_m \in \Ainv$, then $ \varphi_t(\om_m, \hat{A}^m_t(\om)\hat{v}) = \varphi_{t,N} (\om_m, \hat{A}^m_t(\om)\hat{v})$. 
%If $\om_m \in \Asing$, then the equality does not hold only if $\varphi_t(\om_m, \hat{A}^m_t(\om)\hat{v}) < -N$, which is the case when $(t,\hat{v}) \in P_{\varphi,m,N}(\om)$.
%
%Let $B_{\varphi,n,N}(\om) \colon = \cup^{n-1}_{m=0} P_{\varphi,m,N}(\om)$.
%
%Then $\tilde{\eta}(B_{\varphi,n,N}(\om)) \lesssim n^2e^{-N}$ and outside of it both $\varphi_{t}(\om, \hat{A}^n_t(\om)\hat{v}) = \varphi_{t,N}(\om, \hat{A}^n_t(\om)\hat{v}) $ and $S_n \varphi_t = S_n \varphi_{t,N}$.
%
%The proof of the second statement is analogous. Moreover, $B_{\psi,n,N}(\om) \subset B_{\varphi,n,N}(\om)$.
%
%\end{proof}

\subsection{Large deviations estimates}
In order to prove large deviations estimates for cocycles $A\in\cocycles$, we use the following abstract recent result of Cai, Duarte, Klein~\cite[Theorem 1.1.]{CDK-paper3}. Let $\{Z_n\}_{n\ge 0}$ be a Markov chain with values in a compact space $M$, and transition kernel $M\ni x \mapsto K_x \in \Prob (M)$. Let $Q_K \colon L^\infty (M) \to L^\infty (M)$ be the Markov operator corresponding to this kernel, namely $Q_K \phi (x) = \int_M \phi (y) d K_x (y)$. If the operator $Q_K$ is strongly mixing (in an appropriate sense) on some subspace of observables $(\Ecal, \norm{\cdot}_\Ecal)$, relative to a stationary measure $\eta$, then every observable in this subspace $\Ecal$ satisfies (exponential) large deviations. More precisely,  for all $n \ge 1$ consider the $n$-th stochastic sum
$$S_n \phi := \phi \circ Z_{n-1} + \cdots + \phi \circ Z_0 .$$    

Then for all $\ep > 0$, 
\begin{equation}\label{ldt abstract eq}
\Pp \left\{ \abs{ \frac{1}{n} S_n \phi - \int_M \phi \, d\eta } >\epsilon \right\} \le 8e^{-c(\epsilon) n}
\end{equation}
where $c (\ep)$ is an explicit rate function. This rate function is essentially of order $c (\ep) \sim \ep^2 \, \norm{\phi}_\Ecal^{-2}$. See~\cite{CDK-paper3} for more details, specifically Definition 1.1, Theorem 1.1, Remark 1.1. 
In this current work, the Markov operator $\bar \Qop$ is strongly mixing on the entire space of observables $L^\infty (\Ascr \times \Pp^1$ and relative to the $L^\infty$-norm.  
Moreover, for the remaining part of the argument,  it is crucially  important to note the precise dependence of the large deviations estimate on the norm (in our case the $L^\infty$-norm) of the observable. 

We are ready to state and prove a stronger, parametric version of the large deviations type (LDT) estimate for cocycles in $\cocycles$, which will also imply the result stated in the introduction. 



\begin{theorem} 
\label{Parametric LDT} 
Let $A \colon \Lambda \to \cocycles$ be a smooth family of cocycles satisfying Assumptions~\ref{assumptions}.
Then for every $\ep>0$ and $\tilde{\eta}$-a.e $(t,\hat{v})$, there exist $c_0 (\ep) > 0$ and $n_0 (\ep, t,\hat{v}) \in \N$ such that for every $n \geq n_0 (\ep, t, \hat v)$, 
$$
\mu \left\{ \om \in X \colon \abs{  \frac{1}{n} \log \norm{A_t^n (\om) v}  - L_1 (A_t)} >\ep   \right\} < e^{-c_0 (\ep) n^{1/3}} \, .
$$
Moreover, for Lebesgue a.e. $t \in \Lambda$, given any $\ep > 0$ there are $c_0 (\ep) > 0$ and $n_0 (\ep, t) \in \N$ such that for all $n\ge n_0 (\ep, t)$.
 $$
\mu \left\{ \om \in X \colon \abs{  \frac{1}{n} \log \norm{A_t^n (\om) }  - L_1 (A_t)} >\ep   \right\} < e^{-c_0 (\ep) n^{1/3}} \, ,
$$
that is, a (sub-exponential) large deviations type estimate holds for Lebesgue almost every cocycle along the curve $t \mapsto A_t$.
\end{theorem}

\begin{proof}
Given a parameter $t\in\Lambda$, consider the Markov chain $Z_n \colon X \times \Pp^1 \to \Ascr \times \Pp^1$,
$$Z_n (\om, \hat v) := (\om_{n+1}, \hat A_t^n (\om) \hat v) \, .$$

It is easy to see that its transition kernel is given by
$$\Ascr \times \Pp^1 \ni (\om_1, \hat v) \mapsto p \times \delta_{\hat A_t (\om_1) \hat v} ,$$
so that its corresponding Markov operator is precisely the operator $\bar \Qop_t$ defined above, whose stationary measure is $p \times \eta_t$. Recall that by Corollary~\ref{cor strong mixing}, $\Qop_t$ is strongly mixing on $(L^\infty (\Ascr \times \Pp^1), \norm{\cdot}_\infty)$. 

For the observable $\varphi_t(i,\hat{v}) := \log \norm{A_t(i) \frac{v}{\norm{v}}}$ we have that 
\begin{align*}
\varphi_t \circ Z_{n-1} (\om, \hat v) = \varphi_t (\om_n, \hat A_t^{n-1} (\om) \hat v) 
& = \log \norm{  A_t (\om_n) \, \frac{ \hat A_t^{n-1} (\om) \hat v }{\norm{  \hat A_t^{n-1} (\om) \hat v }  }   } \\
& = \log \norm{ \hat A_t^{n} (\om) \hat v }  -  \log \norm{ \hat A_t^{n-1} (\om) \hat v }   \, .
\end{align*}
Thus
$$\frac{1}{n} \, S_n \varphi_t (\om, \hat v) =  \frac{1}{n} \log \norm{A_t^n (\om) v} $$
where $v$ is a unit vector representative of the point $\hat v$.

Moreover, by Furstenberg's formula~\eqref{F formula 10},
$$L_1 (A_t) = \int \psi_t (\hat v) \, d \eta_t (\hat v) = \int \varphi_t (i, \hat v) \, d (p\times\eta_t) (i, \hat v) .$$
It is not difficult to verify  that Lemma~\ref{lem exp small measure} item (iii) implies that for Lebesgue a.e. $t\in\Lambda$, $L_1 (A_t) > - \infty$.

Our statement (in fact, a stronger version thereof) would then immediately follow  from~\eqref{ldt abstract eq} if the observable $\varphi_t$ were bounded. That is of course not the case, precisely because of the singular matrices. The idea is then to use the truncations $\varphi_{t, N}$ (for which estimate~\eqref{ldt abstract eq} is applicable) as a substitute for $\varphi_t$, where the order $N$ of the truncation is adapted to the scale $n$ at which we prove the LDT estimate.  

\smallskip

More precisely, given any large enough scale $n\in\N$, let $N_n \in \N$ be a truncation order to be chosen later (anticipating, the choice that optimizes the estimates will turn out to be $N_n \sim n^{1/3}$). We will transfer the LDT estimate at scale $n$  from $\varphi_{t, N_n}$  to $\varphi_t$ by eliminating an $\tilde \eta$-negligible set of parameters $(t, \hat v)$. 

For all $n\in \N$, define the following real-valued functions on $X \times \Lambda \times \Pp^1$:
\begin{align*}
\Delta_n (\om, t , \hat v) & := \frac{1}{n} S_n \varphi_t (\om, \hat v) - \int  \varphi_t \, d p \times \eta_t  \\
E_n (\om, t , \hat v) & := \frac{1}{n} S_n \varphi_{t, N_n} (\om, \hat v) - \int  \varphi_{t, N_n} \, d p \times \eta_t
\end{align*}
and 
$$g_n (\om, t, \hat v) := \frac{1}{n} S_n \varphi_t (\om, \hat v) - \frac{1}{n} S_n \varphi_{t, N_n} (\om, \hat v) .$$

Then
\begin{equation}\label{super duper eq}
\abs{ \Delta_n (\om, t , \hat v)  - E_n (\om, t , \hat v)  } \le \abs{ g_n (\om, t, \hat v) } + \int  \abs{ \varphi_t - \varphi_{t, N_n} } \, d p \times \eta_t . 
\end{equation}

Note that 
$$\Delta_n (\om, t , \hat v)  = \frac{1}{n} \log \norm{A_t^n (\om) v} - L_1 (A_t) \, .$$

Moreover, given $\ep > 0$, the general LDT estimate~\eqref{ldt abstract eq} and the comments following it show that  {\em for every} $(t, \hat v) \in \Lambda \times \Pp^1$, 
\begin{equation}\label{ldt truncation}
\mu \left\{ \om \in X \colon \abs{ E_n (\om, t , \hat v) } > \frac \ep 2 \right\} \le 8  \, e^{- c_0 (\ep) N_n^{-2} \, n}
\end{equation}
where $c_0 (\ep)$ is essentially of order $\ep^2$.

\smallskip

Using Lemma~\ref{lemma Estimates phi and psi} we have
\begin{align*}
&\int \left(  \int  \abs{ \varphi_t - \varphi_{t, N_n} } \, d p \times \eta_t \right) \, dt \\
&= \sum_{i\in\Ascr} p_i \int_{\Lambda} \int_{\Pp^1} \abs{ \varphi_t (i,  \hat v) -  \varphi_{t, N_n} (i,  \hat v)} \, d\eta_t (\hat{v}) \, dt \less e^{-N_n/3} \, .
\end{align*}

Moreover, we will also show that 
\begin{equation}\label{eq 101010}
\iint \abs{ g_n (\om, t, \hat v) } \, d \mu (\om) \, d \tilde \eta (t, \hat v) \less \sqrt{n} \, e^{-N_n/3} \, .
\end{equation}

Indeed, note that 
$$g_n (\om, t, \hat v) = \frac{1}{n} \sum_{j=1}^{n} \left( \varphi_t (\om_j, \hat A_t^{j-1} (\om) \hat v) -  \varphi_{t, N_n} (\om_j, \hat A_t^{j-1} (\om) \hat v) \right) \, .$$

Given $\om\in X$, if $g_n (\om, t, \hat v) \neq 0$ then there is $1\le j \le n$ such that $\varphi_t (\om_j, \hat A_t^{j-1} (\om) \hat v) \neq  \varphi_{t, N_n} (\om_j, \hat A_t^{j-1} (\om) \hat v)$, that is, $\varphi_t (\om_j, \hat A_t^{j-1} (\om) \hat v) < - N_n$, or $(t, \hat v) \in P_{\om_j, j-1, N_n} (\om)$. 

Thus for $(t, \hat v) \notin B_n (\om) := \bigcup_{j=1}^n P_{\om_j, j-1, N_n} (\om)$, where $\tilde \eta (B_n (\om) \less n e^{- N_n}$, we have that $g_n (\om, t, \hat v) = 0$. 

Using Fubini and Cauchy-Schwarz it follows that
\begin{align*}
& \iint \abs{ g_n (\om, t, \hat v) } \, d \mu (\om) \, d \tilde \eta (t, \hat v) 
 = \iint \abs{ g_n (\om, t, \hat v) } \, d \tilde \eta (t, \hat v) \, d \mu (\om) \\
& = \iint \abs{ g_n (\om, t, \hat v) } \, \ind_{B_n (\om)} (t, \hat v) \, d \tilde \eta (t, \hat v) \, d \mu (\om)  \\
& \le \int \norm{g_n (\om, \cdot)}_{L^2 (\tilde \eta)} \, \, \tilde \eta (B_n (\om))^{1/2} \, d \mu (\om) \\
& \less \sqrt{n} \, e^{-N_n/2} \, \int \norm{g_n (\om, \cdot)}_{L^2 (\tilde \eta)} \, d \mu (\om) \, .
\end{align*}

By Lemma~\ref{lem exp small measure} item (iii), for all $\om\in X$, 
$$\int \varphi_t^2 (\om_j, \hat A_t^{j-1} (\om) \hat v) \, d \eta_t (\hat v) \, d t \le C ,$$
so 
$$\norm{ \frac{1}{n} S_n \varphi_t (\om, \hat v) }_{L^2 (\tilde \eta)} \le \sqrt{C} , $$
while $\abs{ \varphi_{t, N_n} (i, \hat w)} \le N$ so
$$\norm{ \frac{1}{n} S_n \varphi_{t, N_n} (\om, \hat v) }_{L^2 (\tilde \eta)} \le N_n .$$

Thus for all $\om \in X$, $\norm{g_n (\om, \cdot)}_{L^2 (\tilde \eta)} \le  \sqrt{C} + N_n$, which then easily implies~\eqref{eq 101010}.

Integrating the inequality~\ref{super duper eq} with respect to $\mu$ and $\tilde \eta$ we obtain
\begin{equation*}\label{super duper eq2}
\iint \abs{ \Delta_n (\om, t , \hat v)  - E_n (\om, t , \hat v)  } \, d \mu (\om) \, d \tilde \eta (t, \hat v) \less \sqrt{n} \, e^{-N_n/3} \, .
\end{equation*}

Applying Chebyshev's inequality to the function 
$$(t, \hat v) \mapsto \int \abs{ \Delta_n (\om, t , \hat v)  - E_n (\om, t , \hat v)  } \, d \mu (\om) ,$$ 
there is a set $\B_n \subset \Lambda \times \Pp^1$ such that $\tilde \eta (\B_n) \less \sqrt{n} \, e^{-N_n/6}$ and if $(t, \hat v) \notin \B_n$ then
 $$\int \abs{ \Delta_n (\om, t , \hat v)  - E_n (\om, t , \hat v)  } \, d \mu (\om) < e^{-N_n/6} \, .$$ 

Since $\sum_{n\ge1} \tilde \eta (\B_n) < \infty$, by Borel-Cantelli, $\tilde \eta$-almost every $(t, \hat v)$ belongs to a finite number of sets $\B_n$. That is, for  $\tilde \eta$-a.e. $(t, \hat v)$ there is $n_0 (t, \hat v) \in \N$ such that for all $n\ge n_0 (t, \hat v)$ we have $(t, \hat v) \notin \B_n$, so 
$$\int \abs{ \Delta_n (\om, t , \hat v)  - E_n (\om, t , \hat v)  } \, d \mu (\om) < e^{-N_n/6} \, .$$ 

Applying again Chebyshev we have that
$$\mu \left\{ \om\in X \colon \abs{ \Delta_n (\om, t , \hat v)  - E_n (\om, t , \hat v)  } > e^{-N_n/12} \right\} 
\le e^{-N_n/12} .$$

We have shown that there is a set $\Omega_n \subset X$ with $\mu (\Omega_n) < e^{-N_n/12}$ such that if $\om \notin \Omega_n$ then
$$ \abs{ \Delta_n (\om, t , \hat v)  - E_n (\om, t , \hat v)  }  < e^{-N_n/12} \le \frac \ep 2 $$
provided $n$ is large enough depending on $(t, \hat v)$ as above and on $\ep$.

\smallskip

Thus if $ \abs{ \Delta_n (\om, t , \hat v)} > \ep$ then either $\om\in\Omega_n$ or  $\abs{ E_n (\om, t , \hat v)} > \frac \ep 2$, the later holding for $\om$ in a set of measure $\le 8  \, e^{- c_0 (\ep) N_n^{-2} \, n}$ by~\eqref{ldt truncation}. 

We conclude that for $\tilde \eta$-a.e.$(t, \hat v)$ and for all $\ep > 0$ there is $n_0 = n_0 (\ep, t, \hat v) \in \N$ such that for all $n\ge n_0$ we have 
$$\mu \left\{ \om \colon \abs{ \Delta_n (\om, t , \hat v)} > \ep \right\} < e^{-N_n/12} + 8  \, e^{- c_0 (\ep) N_n^{-2} n}
<   e^{- c_0 (\ep) \, n^{1/3} }
$$
provided we choose $N_n \sim n^{1/3}$. This establishes the first statement of the theorem.

In particular, by the definition of the measure $\tilde \eta$, for Lebesgue almost every parameter $t\in\Lambda$ and for $\eta_t$-a.e. point $\hat v$  this first statement of the theorem holds, namely
\begin{equation}\label{ldt vectors}
\mu \left\{ \om \in X \colon \abs{  \frac{1}{n} \log \norm{A_t^n (\om) v}  - L_1 (A_t)} >\ep   \right\} < e^{-c_0 (\ep) n^{1/3}} \, .
\end{equation}

The support of the measure $\eta_t$ is the set 
$$\left\{ \hat A_t^n (s\uom) \hat r_s \colon s \in \Asing, \, \uom \in \Ainv^n, \, n\in \N \right\} .$$

There is at least one singular symbol, $s \in \Asing$ and at least one invertible one $i \in \Ainv$. By the positive winding condition,
$$\frac{d}{dt} \hat A_t (i) \, \hat r_s \ge c_0 > 0 ,$$
so $t \mapsto \hat A_t (i) \, \hat r_s$ cannot be constant on a set of positive Lebesgue measure. Therefore 
$\hat A_t (i) \, \hat r_s \neq \hat r_s$ for Lebesgue almost every $t$.

It follows that for Lebesgue almost every $t\in\Lambda$, the support of the measure $\eta_t$ has at least two points, $\hat e_t^1$ and $\hat e_t^2$. Thus~\eqref{ldt vectors} holds for two linearly independent vectors $e_t^1$ and $e_t^2$ so it must hold  with the matrix norm $ \norm{A_t^n (\om)}$, which establishes the second statement of the theorem.
\end{proof}

%In particular, by the definition of the measure $\tilde \eta$, for Lebesgue almost every parameter $t\in\Lambda$, there must exist at least a point $\hat v_t \in \Pp^1$ for which this first statement of the theorem holds, namely
%$$
%\mu \left\{ \om \in X \colon \abs{  \frac{1}{n} \log \norm{A_t^n (\om) v_t}  - L_1 (A_t)} >\ep   \right\} < e^{-c_0 (\ep) n^{1/3}} \, .
%$$
%
%Clearly
%$$  \Big\{ \om \colon  \frac{1}{n} \log \norm{A_t^n (\om)}  <  L_1 (A_t) - \ep   \Big\}
%\subset  \Big\{ \om \colon  \frac{1}{n} \log \norm{A_t^n (\om) v_t}  <  L_1 (A_t) -\ep  \Big\}
%$$
%so
%$$\mu \Big\{ \om \colon  \frac{1}{n} \log \norm{A_t^n (\om)}  <  L_1 (A_t) - \ep   \Big\} < e^{-c_0 (\ep) n^{1/3}} \, .$$

We now derive the version of the LDT estimate stated in the introduction.


\begin{proof}
	[Proof of Theorem~\ref{thm: ldt intro}]
Given $\uA\in \Mat_2(\R)^k$ with $L_1(\uA)>L_2(\uA)$, we consider the following cases:

\noindent 
\blob\; $A_i$ is invertible for all $i=1, \ldots, k$ and $\uA$ or $\uA^{-1}$  is a quasi-irreducible cocycle.
This is  is the classical case  where  E. Le Page
proved,
under a strong irreducibility hypothesis on $\uA$, large deviations of exponential type~\cite[Th\'eor\`{e}me 7]{LP82}.
These large deviations are stable under perturbations of $\uA$, see~\cite[Theorem 5.3]{DK-book}. Stable large deviations of exponential type  under these specific assumptions follow from~\cite[Theorem 1.1]{DK-Holder}.


\noindent 
\blob\; $A_i$ is invertible for all $i=1, \ldots, k$ but  neither $\uA$ nor $\uA^{-1}$  are quasi-irreducible, i.e., $\uA$ is diagonalizable. This is the setting of the main theorem in~\cite{DK-Holder} where stable large deviations of sub-exponential type were established, see \cite[Theorem 1.1]{DK-Holder}.
We can neglect this case because the space of  diagonalizable cocycles is an algebraic variety of positive codimension $2k-2>0$ (when $k>1$) and hence has zero Lebesgue measure.
Notice that this space is the range of the algebraic map
$\GL_2(\R)\times \mathrm{Diag}_2(\R)^k\to \Mat_2(\R)^k$,
$$(S, (D_1, \ldots, D_k))\mapsto \left( S^{-1}\, D_1\, S,\ldots,  S^{-1}\, D_k\, S\right) $$
which has dimension $2+2k$ and codimension $2k-2$ in $\Mat_2(\R)^k$.




\noindent 
\blob\;  $A_i$ is singular (non-invertible) for at least some $i=1, \ldots, k$. Let $\Mscr$ denote the subspace of $\Mat_2(\R)^k$ consisting of all such cocycles and consider the analytic manifolds $\Mscr_I$ introduced in the proof of Theorem~\ref{thm: BM type dichotomy}.
Since $\Mscr\setminus \cup_{|I|>0} \Mscr_I$ has zero Lebesgue measure
we can restrict the proof to the strata $\Mscr_I$. We are going to prove
 more than was stated, namely  that large deviations of exponential type hold for Lebesgue almost every
$\uA$ in $\Mscr_I$.

Given $\uA\in \Mscr_I$ define
$\uA(t):=(A_1(t), \ldots, A_k(t))$, where
$$ A_i(t):= \begin{cases}
	A_i\, R_t & \text{ if }  \, i\in I \\
A_i &\text{ if } \, i\notin I
\end{cases} \quad \text{ and } \quad R_t:= \begin{bmatrix}
\cos t & -\sin t \\ \sin t & \cos t 
\end{bmatrix} . $$
This is an analytic family taking values in $\Mscr_I$ and satisfying the assumptions (A1), (A2) of Section~\ref{StatProp}. By Theorem~\ref{Parametric LDT}, $\uA(t)$ satisfies large deviations of sub-exponential type for Lebesgue almost every $t\in \R$.
Hence, since the map $\Mscr_I\times \R \to \Mscr_I$,
$(\uA, t)\mapsto \uA(t)$, is a submersion, Lebesgue almost every
$\uA\in \Mscr_I$ satisfies similar large deviations estimates.
\end{proof}









\begin{subsection}{Central limit theorem}

We now establish a central limit theorem for singular cocycles.  The proof uses the following abstract central limit theorem~\ref{thm Abstract CLT}  due to Gordin-Liv\v sic~\cite{Go78}.

Let $\varphi \in L^2 (M, \nu)$ be an observable with $\int \varphi \; d\nu =0$. If  $ \sum_{n=0}^\infty \norm{Q^n \varphi}_2 < \infty$ then we can define $g \in L^2(M, \nu)$ by
$$
g := \sum_{n=0}^\infty Q^n \varphi.
$$
Then $\varphi = g - Q g$. Let $\sigma^2(\varphi) = \norm{g}_2^2 - \norm{Q g}^2_2$.

\begin{theorem} \label{thm Abstract CLT} 
(Gordin-Livsic)
Let $(M,Q,\nu)$ be an ergodic Markov system and let $\varphi \in L^2(M)$ with $\int \varphi \; d\nu =0$. Assume that 
$$
\sum_{n=0}^\infty \norm{Q^n\varphi}_2 < \infty \quad \text{and } \sigma^2(\varphi) \in (0,\infty).
$$
Then the following central limit theorem holds:
$$
\frac{S_n\varphi}{\sigma \sqrt{n}} \to \mathcal{N}(0,1).
$$
We note that this result holds not only relative to the Markov probability with initial distribution $\eta$, but also with initial distribution $\delta_x$ for $\nu$-a.e. $x\in M$.
\end{theorem}







We consider as in the previous subsection a smooth family of cocycles $\Lambda \ni t \mapsto \uA_t \in \cocycles$ satisfying the positive winding property. We also consider the special observables $\psi_t$ and $\varphi_t$ from before. 

We introduced two related (families of) Markov operators acting on measurable bounded observables. They can actually be defined for arbitrary observables, namely if $\psi \colon \Pp(\R^2)  \to [-\infty, \infty)$ we put
$$\Qop_t \psi (\hat{v}) = \sum_{i \in \Ascr} p_i \psi(\hat{A}_t(i)\hat{v}) $$
and if $\varphi \colon \Ascr \times \Pp(\R^2)  \to [-\infty, \infty)$ we put
$$\bar{\Qop}_t \varphi(j,\hat{v}) = \sum_{i \in \Ascr}  p_i \varphi(i, \hat{A}_t(j) \hat{v}) .$$

Consider the projection:
\begin{align*}
&\pi \colon L^2(\Ascr \times \Pp(\R^2)) \to L^2(\Ascr) \\ 
& \pi \varphi (\hat{v}) := \sum_{i \in \Ascr} p_i \varphi (i,\hat{v}).
\end{align*} 
Using this notation, $\pi \varphi_t = \psi_t$. Moreover, $\bar{\Qop}^{n+1}_t \varphi(i,\hat{v}) = \Qop^n_t (\pi \varphi)(\hat{A}_t(i)\hat{v})$.





%\begin{theorem} (Gordin-Livsic)
%\label{thm:Gordin-Livsic}
%Let $(M,Q,\nu)$ be an ergodic Markov system. Let $\varphi \in L^2(M)$ with $\int \varphi \; d\nu =0$. Assume that 
%$$
%\sum_{n=0}^\infty \norm{Q^n\varphi}_2 < \infty \quad \text{and } \sigma^2(\varphi) \in (0,\infty).
%$$
%Then,
%$$
%\frac{S_n\varphi}{\sigma \sqrt{n}} \to \mathcal{N}(0,1).
%$$
%\end{theorem}


\begin{lemma} \label{last lemma} For Lebesgue almost every parameter $t\in\Lambda$ we have that
$$
\sum_{n=0}^\infty \norm{ \bar{\Qop}^{n+1}_t\varphi_t - \int \varphi_t \; dp d\eta_t }_{L^2(p \times \eta_t)} < \infty.
$$
\end{lemma}
\begin{proof}
By the previous observations,
\begin{align*}
\sum_{n=0}^\infty \norm{ \bar{\Qop}^{n+1}_t\varphi_t - \int \varphi_t \; dp d\eta_t }_{L^2} &= \sum_{n=0}^\infty \norm{ \Qop^n_t \psi_t(\hat{A}_t(i)\hat{v}) - \int \psi_t \; d\eta_t }_{L^2} \\
&\kern-4em = \sum_{n=0}^\infty \left( \sum_{i \in \Ascr} p_i  \int \left| \Qop^n_t \psi_t(\hat{A}_t(i)\hat{v}) - \int \psi_t \; d\eta_t \right|^2 \; d\eta_t(\hat{v}) \right)^{\frac{1}{2}}.
\end{align*}
%$$
%\sum_{n=0}^\infty \norm{ \Qop^n_t \psi_t(\hat{A}_t(i)\hat{v}) - \int \psi_t \; d\eta_t }_{L^2(\mu \times \eta_t)} < \infty.
%$$
%Moreover, the left hand side is equal to 
We start by showing that for every $i \in \Ascr$ there exists $\sigma \in (0,1)$ such that for every $n \in \N$
$$
\int_{\Lambda} \int_{\Pp(\R^2)}  \left| \Qop^n_t \psi_t(\hat{A}_t(i)\hat{v}) - \int \psi_t \; d\eta_t \right|^2 \; d\eta_t(\hat{v}) \;dt \lesssim \sigma^n.
$$ 
Fix $i \in \Ascr$ and note that by lemma~\ref{lem exp small measure} item (iii) and Jensen's inequality,
\begin{align*}
&\int_{\Lambda} \int_{\Pp(\R^2)}  \left| \Qop^n_t \psi_t(\hat{A}_t(i)\hat{v})  - \int \psi_t \; d\eta_t \right|^2 \; d\eta_t(\hat{v}) \;dt \\
&= \int_{\Lambda} \int_{\Pp(\R^2)} \Big| \sum_{\uom \in \Ainv^n} p(\uom) \psi_t(\hat{A}^n_t(\uom)\hat{A}_t(i)\hat{v}) \\
& - \sum_{s \in \Asing}p_s \sum_{j=n}^\infty \sum_{\uom \in \Ainv^j} p(\uom) \psi_t(\hat{A}_t^j(\uom)r_s)  \Big|^2d\eta_t(\hat{v})dt \\
&\leq 2 \int_{\Lambda} \int_{\Pp(\R^2)} \sum_{\uom \in \Ainv^n} p(\uom) \left| \psi_t(\hat{A}^n_t(\uom)\hat{A}_t(i)\hat{v}) \right| ^2 \; d\tilde{\eta}(t,\hat{v})  \\
&+ 2 \int_{\Lambda} \int_{\Pp(\R^2)} \sum_{s \in \Asing}p_s \sum_{j=n}^\infty \sum_{\uom \in \Ainv^j} p(\uom) \left| \psi_t(\hat{A}_t^j(\uom)r_s) \right| ^2  \; d\tilde{\eta}(t,\hat{v}) \\
&\less \sum_{\uom \in \Ainv^n} p(\uom)  +  \sum_{s \in \Asing}p_s \sum_{j=n}^\infty \sum_{\uom \in \Ainv^j} p(\uom)  \less (1-q)^n 
\end{align*}
so the claim holds with $\sigma=1-q$.

By Chebyshev's inequality, 
$$
\Leb \left\{ t \in \Lambda \colon \int_{\Pp(\R^2)} \left|  \Qop^n_t \psi_t(\hat{A}_t(i)\hat{v}) - \int \psi_t \; d\eta_t  \right|^2 \;d\eta_t (\hat{v}) > \sigma^\frac{n}{2}   \right\} \less \sigma^\frac{n}{2}.
$$

Therefore, for every $i \in \Ascr$ and for each $n \in \N$, there exists a set $B_n(i) \subset \Lambda$, with $\Leb(B_n(i)) \less\sigma^{\frac{n}{2}}$ such that for every $t \notin B_n(i)$,
\begin{equation} \label{Eq Gordin Livsic}
\norm{\bar{\Qop}_t^{n+1} \varphi_t - \int_{\Ascr \times \Pp(\R^2)} \varphi_t \; d p d\eta_t}_{L^2(p \times \eta_t)} \lesssim \sigma^{\frac{n}{2}}.
\end{equation}

Moreover, since there is a finite number of symbols, there exists a set $B_n$ that satisfies the same properties for all symbols $i\in\Ascr$ simultaneously. Furthermore, since $\sum_{n=0}^\infty \Leb(B_n) < \infty$, by the Borel-Cantelli lemma, for almost every $t \in \Lambda$, there exists $n_0(t) \in \N$ such that for every $n \geq n_0(t)$, $t \notin B_n$. Thus for almost every $t$, the inequality \eqref{Eq Gordin Livsic} holds, hence
$$
\sum_{n=0}^\infty \norm{ \bar{\Qop}^{n+1}_t\varphi_t - \int \varphi_t \; d p d\eta_t }_{L^2(p \times \eta_t)} < \infty.
$$
which proves the lemma.
\end{proof}



\medskip

We are ready to formulate and to prove a parametric version of the CLT for singular cocycles. 

\begin{theorem}
\label{Parametric CLT}
For almost every $t \in \Lambda$ there exists $\sigma=\sigma(t)>0$ such that the following convergence in distribution holds:
$$
\frac{\log \norm{A_t^n}-n\, L_1(A_t)}{\sigma\, \sqrt{n}} \stackrel{d}{\to} \mathcal{N}(0,1).
$$
%Moreover, for Lebesgue almost every $\hat v\in \Pp(\R^2)$, and also for $\eta_t$-a.e. $\hat v\in \Pp(\R^2)$,
%$$
%\frac{\log \norm{A_t^n\, v}-n\, L_1(A_t)}{\sigma\, \sqrt{n}} \stackrel{d}{\to} \mathcal{N}(0,1) .
%$$
\end{theorem}

\vspace{-1em}

\begin{proof}
 In order to apply theorem~\ref{thm Abstract CLT}  and establish the central limit theorem, we first note that for every parameter $t$, the Markov system $(\Ascr\times\Proj(\R^2), \bar \Qop_t)$  is ergodic, since it has a unique stationary measure $p \times \eta_t$. That is because $\bar{\Qop}^n_t \varphi \to \int \varphi \; d p d\eta_t$ uniformly for every $\varphi \in L^\infty(\Ascr \times \Pp(\R^2))$. 
 %Hence, if $\nu_t$ is $\bar{\Qop}$-stationary, then 
% $$
% \int \varphi \; d\nu_t = \int \bar{\Qop}^n \varphi \; d\nu_t \to \int \varphi \; d\mu d\eta_t.
% $$ 
% Thus, we conclude that $\nu_t = \eta_t$.
 
 Consider the special observable $\varphi_t$ defined before and recall from the previous lemma that for Lebesgue almost every parameter $t\in\Lambda$ we have  
 $$\sum_{n=0}^\infty \norm{ \bar{\Qop}^{n}_t\varphi_t - \int \varphi_t \; dp d\eta_t }_{L^2(p \times \eta_t)} < \infty .$$  
 
This in particular allows us to define
$$
g_t := \sum_{n=0}^\infty \bar{\Qop}^n_t \left(\varphi_t - \int \varphi_t \; dp d\eta_t\right) \in L^2 (p\times\eta_t) .
$$

Then  for every parameter $t$,
$$\varphi_t - \int \varphi_t \; dp d\eta_t = g_t - \bar{\Qop}_t g_t .$$
 
 Let $\sigma^2 (t) = \sigma^2_t(\varphi_t) := \norm{g_t}_2^2 - \norm{\bar{\Qop}_t g_t}^2_2$.
 
 \medskip

Hence in order to apply theorem~\ref{thm Abstract CLT}  it remains to prove that $\sigma^2 (t)>0$ for almost every $t \in \Lambda$. 
%In fact, it is true for every $t \in \Lambda.$
%It remains to verify that $\sigma^2(\varphi) \in (0,\infty)$. In order to verify this fact, we use proposition $2.2$ of 
%{\color{blue} cite paper 3 CDK}. In fact, we already know that $\Qop^n \varphi \to \int \varphi \; d\mu d\eta$ uniformly for every continuous $\varphi$. 

This is established in the next lemma by adapting the proof of~\cite[proposition 2.2]{CDK-paper3}, which is a version of the abstract CLT of Gordin-Liv\v sic  more immediately applicable to dynamical systems.
%Finally we prove that\, 
	%$\sigma^2(\varphi)>0.$

\begin{lemma}The variance-type quantity defined above satisfies 
$\sigma^2(t)>0$ for every $t \in \Lambda$.
\end{lemma}
\begin{proof}
Consider the family of Markov operators $\bar{\Qop}_t \colon L^\infty(\Ascr \times \Pp(\R^2)) \to L^\infty(\Ascr \times \Pp(\R^2)) $, given by $(\bar{\Qop}_t \varphi)(j,\hat v) = \sum_{ i\in\Ascr}  \varphi(i,\hat A_t(j)\, \hat v)\, p_{i}$ and the corresponding family of Markov kernels $\bar{K}_t \colon (\Ascr \times \Pp(\R^2)) \to \Prob(\Ascr \times \Pp(\R^2))$. Recall that the measure $p \times \eta_t$ is $\bar{K}_t$-stationary, in the sense that $(\bar{K}_t)_* p \times \eta_t =p \times  \eta_t$.
	
%Moreover, note that theorem~\ref{Uniform Ergodicity} is valid  for every bounded observable. Thus, $p \times \eta_t$ is the unique $\bar{K}_t$-stationary measure and for each $t$, the Markov system $(\Ascr \times \Pp(\R^2), \bar{K}_t, p \times \eta_t)$ is ergodic.
%	
%	Note that it suffices to prove the result for the observable $\tilde{\varphi} = \varphi - \int \varphi \; d p \times \eta_t$, which satisfies $\int \tilde{\varphi} \;dp \times \eta_t =0$. By an abuse of notation, in this proof we will use $\varphi$ to denote $\tilde{\varphi}$.
	
	Fix any $t \in \Lambda$. Assume by contradiction that $\sigma_t^2(\varphi)=0$. 
	Let $x,y \in \Ascr \times \Pp(\R^2)$ with $x=(i,\hat{v}_1)$ and $y = (j,\hat{v}_2)$.
	Then
	\begin{align*}
		0 &\leq \int (\bar{\Qop}_t \, g_t (x) - g_t(y))^2 \; d\bar{K}_{t,x}(y) dp \times \eta_t(x) \\
		&= \int \left\{ (\bar{\Qop}_t \, g_t (x))^2 + (g_t(y))^2 -2 g_t(y)\bar{\Qop}_t g_t (x)\right\} \; d\bar{K}_{t,x}(y) dp \times \eta_t(x) \\
		& = \int \left\{   (g_t(y))^2 - (\bar{\Qop}_t \, g_t (x))^2\right\} \; d\bar{K}_{t,x}(y) dp \times \eta_t(x) \\
		&=\norm{g_t}_2^2 - \norm{\bar{\Qop}_t \, g _t}_2^2 = \sigma^2 (t) = 0.
	\end{align*}
	
We then conclude that $g_t(y) = \bar{\Qop}_t g_t(x)$ for $p \times \eta_t$-a.e $x$ and $\bar{K}_{t,x}$-a.e $y$. By induction, for every $n \geq 1$
	$ \bar{\Qop}_t^n g_t(x) = g_t(y) $ for $p \times \eta_t$-a.e $x$ and $\bar{K}_{t,x}^n$-a.e $y$. Hence for all $n \geq 1$ and $p \times \eta_t$-a.e $x$, $g_t$ is $\bar{K}^n_{t,x}$-a.e constant. 
	
	We claim that in fact $g_t$ is $p \times \eta_t$-a.e constant. Assume by contradiction that $g_t$ is not constant for $p \times \eta_t$-a.e. Then there exist two points $x_1$ and $x_2$ in the support of the stationary measure $p \times \eta_t$ such that $p \times \eta_t(\{ x_1\})>0$, $p \times \eta_t(\{ x_2 \})>0$ and $g_t|_{ \{ x_1 \} } < g_t|_{ \{ x_2 \} }$.
	Define $\phi_1 =  \mathbbm{1}_{\{ x_1 \}}$ and $\phi_2 = \mathbbm{1}_{\{ x_2 \}}$. Note that $0 \leq \phi_i = \mathbbm{1}_{\{ x_i \}}$ and $\int \phi_i \; dp \times \eta_t>0$ for $i=1,2$. Moreover, for every $x \in \Ascr \times \Pp(\R^2)$ and every $n \geq 1$, uniformly in $x$ we have
	$$
	\bar{K}_{t,x}^n(\{ x_i \})=(\bar{\Qop}_t^n \mathbbm{1}_{\{ x_i \}}) (x) = (\bar{\Qop}_t^n \phi_i)(x) \to \int \phi_i \; dp \times \eta_t>0 . 
	$$

Then for $n$ sufficiently large and for every $x \in \Ascr \times \Pp(\R^2)$, $\{x_1\}$ and $\{x_2\}$ have positive $\bar{K}_{t,x}^n$ measure. However, $g_t|_{\{ x_1\} } < g_t|_{\{ x_2\} }$, contradicting the fact that $g_t$ is $\bar{K}_{t,x}^n$-a.e constant for $p \times \eta_t$-a.e $x$. Thus, $g_t$ is $p \times \eta_t$-a.e constant.
Since $\bar{\Qop}_t$ preserves constants, it follows that $\varphi_t = g_t - \bar{\Qop}_t g_t =0 \; \; p \times \eta_t$-a.e. which, however, cannot hold. We obtained a contradiction, so $\sigma^2 (t) > 0$ as stated. 
\end{proof}

Theorem~\ref{thm Abstract CLT} is then applicable to the Markov system $(\Ascr\times\Proj(\R^2), \bar K_t)$ and the observable $\varphi_t$, for Lebesgue almost every $t\in\Lambda$. We then conclude that for $\eta_t$-a.e. point $\hat v \in \Proj (\R^2)$, 
$$
\frac{\log \norm{A_t^n\, v}-n\, L_1(A_t)}{\sigma\, \sqrt{n}} \stackrel{d}{\to} \mathcal{N}(0,1) .
$$

As in the proof of the large deviations estimate, the support of the measure $\eta_t$ has at least two points, so the convergence above holds for at least two linearly independent vectors. Then it must hold with the matrix norm:
$$
\frac{\log \norm{A_t^n}-n\, L_1(A_t)}{\sigma\, \sqrt{n}} \stackrel{d}{\to} \mathcal{N}(0,1) ,
$$
which concludes the proof of the theorem.
\end{proof}

We note that the non-parametric version of the CLT stated in the introduction, namely theorem~\ref{thm: clt intro}, can be derived form the parametric version exactly the same way the non-parametric LDT theorem~\ref{thm: ldt intro} was derived from the parametric LDT theorem~\ref{Parametric LDT}. Thus theorem~\ref{thm: clt intro} holds as well.

%\begin{proof}
	%[of Theorem~\ref{thm: clt intro}]
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Given $\uA\in \Matdm^k$ with $L_1(\uA)>L_2(\uA)$, we consider the same  cases as in the  proof above:
%
%\noindent 
%\blob\; $A_i$ is invertible for all $i=1, \ldots, k$ and $\uA$ or $\uA^{-1}$  is a quasi-irreducible cocycle.
%This is  is the classical case  where  E. Le Page
%proved,
%under a strong irreducibility hypothesis on $\uA$, a CLT~\cite[Th\'eor\`{e}me 2]{LP82}.
%The CLT  under our specific assumptions holds with the same
%spectral proof' strategy. Alternatively it holds because the  quasi-irreducibility of $\nu$ and the gap $L_1(\nu)>L_2(\nu)$ imply a strong mixing property with exponential decay rate which in turn imply that the main hypothesis of the abstract CLT of Gordin-Livsic (Theorem \ref{thm:Gordin-Livsic}) holds.
%
%\noindent 
%\blob\; The case when $A_i$ is invertible for all $i=1, \ldots, k$ but  neither $\uA$ nor $\uA^{-1}$  are quasi-irreducible can be neglected  because the space of  these cocycles is an algebraic variety of positive codimension  and hence has zero Lebesgue measure.
% 
%
%\noindent 
% $A_i$ is singular (non-invertible) for at least some $i=1, \ldots, k$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The proof of this theorem is the same as in  Theorem~\ref{thm: ldt intro}, using Theorem~\ref{Parametric CLT} instead of  Theorem~\ref{Parametric LDT}.
%\end{proof}

\begin{remark}\label{ldt-clt rank=1}
Projectively uniformly hyperbolic cocycles automatically satisfy uniform LDT estimates and a CLT, since these properties  can be immediately reduced to the corresponding limit laws for i.i.d. additive processes in classical probabilities. In particular, by Theorem~\ref{ManeBochiRank1}, if all components of $\uA \in \Mat_2 (\R)^k$ are singular and $L_1 (\uA) > - \infty$ then $\uA$ satisfies uniform LDT estimates and a CLT.
\end{remark}
\end{subsection}


\begin{remark}\label{ldt-clt rank=1}
Projectively uniformly hyperbolic cocycles automatically satisfy uniform LDT estimates and a CLT, since these properties  can be immediately reduced to the corresponding limit laws for i.i.d. additive processes in classical probabilities. In particular, by Theorem~\ref{ManeBochiRank1}, if all components of $\uA \in \Mat_2 (\R)^k$ are singular and $L_1 (\uA) > - \infty$ then $\uA$ satisfies uniform LDT estimates and a CLT.
\end{remark}
